A Fast Algorithm for Computing the Deficiency Number of a Mahjong Hand

The tile-based multiplayer game Mahjong is widely played in Asia and has also become increasingly popular worldwide. Face-to-face or online, each player begins with a hand of 13 tiles and players draw and discard tiles in turn until they complete a winning hand. An important notion in Mahjong is the deficiency number (a.k.a. shanten number in Japanese Mahjong) of a hand, which estimates how many tile changes are necessary to complete the hand into a winning hand. The deficiency number plays an essential role in major decision-making tasks such as selecting a tile to discard. This paper proposes a fast algorithm for computing the deficiency number of a Mahjong hand. Compared with the baseline algorithm, the new algorithm is usually 100 times faster and, more importantly, respects the agent's knowledge about available tiles. The algorithm can be used as a basic procedure in all Mahjong variants by both rule-based and machine learning-based Mahjong AI.

==> experiments.tex <==
%
\lsj{Demonstrate the merits of the new deficiency calculating method by experiments: }

\lsj{Describe how the test data is generated. The data can be classified into three categories according to the number (1, 2, or 3) of different colour a hand may have.  Compare with the quadtree method, how efficient it is? Compare with the approximate quadtree method, how precise it is?}
\begin{itemize}
    \item 100x fast than the basic method.
    \item Can use the better discard method.
    \item Can be used to generate more game records.
\end{itemize}

To illustrate the performance of the proposed block algorithm, several experiments are designed and conducted in  this section. In particular, the efficiency of the block algorithm is verified by counting and comparing the number of the type with that of the {\qd} for various cases, and three type of hands are employed to demonstrate the merit of the block algorithm by comparing with the quandtree algorithm.  Moreover, to have statistically sound conclusions, the Wilcoxon signed rank test is further employed to show the differences between the block algorithm and the quandtree algorithm on their search time.


\subsection*{6.1 The efficiency of the block algorithm}

In this subsection, the efficiency of the block algorithm is illustrated by comparing the number of the type with that of {\qd} on the various blocks, and the proposed block algorithm with the quandtree algorithm on the various hands, respectively.


\subsubsection*{6.1.1 The comparison of the type and {\qd} on the various blocks}

First, to constitutionally show the efficiency of the block algorithm, the number of the type and that of {\qd} on the various blocks are counted and compared. Obviously, the type of one block is employed to calculate the deficiency of the corresponding hand, so the number of the type could accurately reflect the efficiency of the proposed block algorithm. Thus, this experiment is reasonable and valid. Specially, to effectively avoid the randomness of the experimental result, all blocks with different number of the tile (2 to 14) are used to test, and each block are tested simultaneously with a deterministic knowledge base and a random knowledge base. Herein, the deterministic knowledge base means that the knowledge base is consisted of the all remaining tiles for the current block, and the random knowledge base means that each element of the knowledge base is randomly generated within the number of the corresponding element of the deterministic knowledge base. Table \ref{tab1} shows the average number of the type and {\qd} for each type of block under the above two knowledge bases.

From Table \ref{tab1}, one can see that the average number of the type is always less than that of {\qd} in all cases. In particular, for the blocks with the deterministic knowledge base, when the size of block is 6, 7, and 10-14, the average number of the corresponding type is less than that of {\qd} with one order of magnitude. Meanwhile, for the blocks with the random knowledge base, when the size of block is 6 and 10-14, the average number of the corresponding type is also less than that of {\qd} with one order of magnitude. Moreover, to further demonstrate the difference between the average number of the type and that of {\qd} and investigate the relationship between the average number of the type and {\qd} and the size of the block, Figure \ref{fig1} depicts the changing curves of the average number of the type and {\qd} with various block sizes under the different knowledge bases. From Figure \ref{fig1}, we can see that whenever under the deterministic knowledge base and the random one, the average number of the type is always less than that of {\qd}, and their average number is more and more large with the increasement of the size of block. The reason for these might be that as the number of the tile in block is larger, the number of the valid different combinations among them will be naturally more. Thus, the proposed block algorithm has a faster search efficiency.


\begin{table}
\begin{center}
\caption{\label{tab1} The average number of the type and {\qd} on the blocks with various sizes}
\scalebox{0.60}[0.75]{
\begin{tabular}{|c| c| c| c| c|}
\noalign{\vskip 1mm}
\hline
	&\multicolumn{2}{c|}{Deterministic knowledge base}	&\multicolumn{2}{c|}{Random knowledge base}		\\
\hline Block size	&The average number of qDCMPs	&The average number of types	&The average number of qDCMPs	&The average number of types\\
\hline 2	&$2.00 \times 10^0$ &$2.00 \times 10^0$	 &$2.04 \times 10^0$    &$1.88 \times 10^0$\\
\hline 3	&$3.10 \times 10^0$	&$2.73 \times 10^0$  &$2.90 \times 10^0$	&$2.83 \times 10^0$\\
\hline 4	&$5.38 \times 10^0$	&$4.30 \times 10^0$	 &$4.97 \times 10^0$	&$4.70 \times 10^0$\\
\hline 5	&$9.10 \times 10^0$	&$6.14 \times 10^0$	 &$8.24 \times 10^0$	&$6.64 \times 10^0$\\
\hline 6	&$1.57 \times 10^1$	&$8.77 \times 10^0$	 &$1.40 \times 10^1$	&$9.95 \times 10^0$\\
\hline 7	&$2.69 \times 10^1$	&$1.23 \times 10^1$	 &$2.36 \times 10^1$	&$1.41 \times 10^1$\\
\hline 8	&$4.67 \times 10^1$	&$1.71 \times 10^1$	 &$3.99 \times 10^1$	&$2.00 \times 10^1$\\
\hline 9	&$8.14 \times 10^1$	&$2.35 \times 10^1$	 &$6.89 \times 10^1$	&$2.79 \times 10^1$\\
\hline 10	&$1.43 \times 10^2$	&$3.24 \times 10^1$	 &$1.19 \times 10^2$	&$3.89 \times 10^1$\\
\hline 11	&$2.53 \times 10^2$	&$4.39 \times 10^1$  &$2.07 \times 10^2$	&$5.30 \times 10^1$\\
\hline 12	&$4.50 \times 10^2$	&$5.96 \times 10^1$	 &$3.63 \times 10^2$	&$7.15 \times 10^1$\\
\hline 13	&$8.03 \times 10^2$	&$7.96 \times 10^1$	 &$6.39 \times 10^2$	&$9.44 \times 10^1$\\
\hline 14	&$1.44 \times 10^3$	&$1.05 \times 10^2$	 &$1.13 \times 10^3$	&$1.23 \times 10^2$\\
\hline
\end{tabular}}
\end{center}
\end{table}

\begin{figure}
  \centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=12cm]{fig_log_0.png}\\
  \caption{The relationship between the average number of the type and {\qd} with the various block sizes }\label{fig1}
\end{figure}




\subsubsection*{6.1.2 The comparison of the block algorithm and the quandtree algorithm on the various hands} 


Moreover, to wholly evaluate the efficiency of the block algorithm, the type in the block algorithm is further compared with the {\pd} in the quadtree algorithm on the various hands. Due to the fact that the types of the various combinations and the {\pd}s generated by the search process are respectively used to calculate the deficiency in the block algorithm and the quadtree algorithm, then the number of the types and {\pd}s could be reasonably considered as their efficiency for one hand. In particular, to ensure the accuracy of the comparison results, two different types of hands, {\sl i.e.}, with two and three colours, are simultaneously employed to test, and each corresponding experiment contains all hands with different number of blocks. It should be noted that since the test of the hands with one colour is the same as in the last subsections, the corresponding experiments would be not conducted here once more.  Tables \ref{tab2} and \ref{tab3} show the average number of the types in the block algorithm and {\pd}s in the quadtree algorithm on the hands with two and three colours, respectively.

\begin{table}
\begin{center}
\caption{\label{tab2} The average number of the types in the block algorithm and {\pd}s in the quadtree algorithm on the hands with two colours}
\scalebox{0.75}[0.85]{
\begin{tabular}{|c| c| c| c| c| c| c| c|}
\noalign{\vskip 1mm}
\hline
The number of block	&The number of hand	&The average number of {\pd}s	&The average number of types \\
\hline 2	&2212	&$5.70 \times 10^2$	&$3.36 \times 10^1$ \\
\hline 3	&4918	&$4.52 \times 10^2$	&$3.61 \times 10^1$ \\
\hline 4	&2528	&$3.69 \times 10^2$	&$4.00 \times 10^1$ \\
\hline 5	&331	&$2.94 \times 10^2$	&$3.92 \times 10^1$ \\
\hline 6	&11	    &$2.49 \times 10^2$	&$3.64 \times 10^1$ \\
\hline
\end{tabular}}
\end{center}
\end{table}

\begin{table}
\begin{center}
\caption{\label{tab3} The average number of the types in the block algorithm and {\pd}s in the quadtree algorithm on the hands with three colours}
\scalebox{0.75}[0.85]{
\begin{tabular}{|c| c| c| c| c| c| c| c|}
\noalign{\vskip 1mm}
\hline
The number of block	&The number of hand	&The average number of {\pd}s	&The average number of types\\
\hline 3	&546	&$3.99 \times 10^2$	&$2.75 \times 10^1$ \\
\hline 4	&2389	&$2.96 \times 10^2$	&$2.80 \times 10^1$ \\
\hline 5	&3646	&$2.16 \times 10^2$	&$2.71 \times 10^1$ \\
\hline 6	&2591	&$1.52 \times 10^2$	&$2.30 \times 10^1$ \\
\hline 7	&724	&$1.03 \times 10^2$	&$1.82 \times 10^1$ \\
\hline 8	&102	&$6.98 \times 10^1$	&$1.48 \times 10^1$ \\
\hline 9	&2	    &$5.60 \times 10^1$	&$1.00 \times 10^1$ \\
\hline
\end{tabular}}
\end{center}
\end{table}


From Tables \ref{tab2} and \ref{tab3}, we can see that the average number of the types in the block algorithm is always less than that of {\pd}s in the quadtree algorithm in all cases. In particular, for the hands with two colours, the average number of the types is less than that of {\pd}s with one order of magnitude in all cases; and for the hands with three colours, when the number of the block is 3-7, the average number of the types is less than that of {\pd}s with one order of magnitude in all cases. Moreover, to clearly illustrate the difference between the the block algorithm and the quadtree algorithm, and the influence of the number of the block for the average number of the types and {\pd}s, Figures \ref{fig2}-\ref{fig3} depict the changing curves between the average number of the types and {\pd}s and the block size on the hands with two and three colours, respectively. From Figures \ref{fig2}-\ref{fig3}, we can see that the average number of the types is always less than that of {\pd}s on both the hands with three colours and those with two colours, and as the number of block increases, the number of the types and {\pd}s gradually reduces. These might be attributed to the fact that as the number of block increases, the number of the tile in each block will be reduced and the tiles in the hand are more scattered, such that the number of the possible types in each block and that of the possible {\pd}s is smaller, which would then lead to the less number of the types and {\pd}s. Therefore, the proposed block algorithm is more efficient than the quadtree algorithm.



\begin{figure}
  \centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=12cm]{exp2_2color.png}\\
  \caption{The changing curve between the average number of the types and {\pd}s and the block size on the hand with two colours}\label{fig2}
\end{figure}


\begin{figure}
  \centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=12cm]{exp2_3color.png}\\
  \caption{The changing curve between the average number of the types and {\pd}s and the block size on the hand with three colours}\label{fig3}
\end{figure}



\subsection*{6.2 The performance of the block algorithm}

In this subsection, the performance of the block algorithm is shown by several experiments on various types of hands, including the hands with one colour, the hands with two colours and the hands with three colours. In particular, to effectively avoid the randomness of the test and other disturbances, 1000 random hands with different 30 random knowledge bases and 100 random knowledge bases are respectively used for the above three types hands, while each hand is repeatedly tested with 10 times, and the success ratio of the search results and the average search time of the ten runs are adopted to measure the performance of the algorithm. Furthermore, to have statistically sound conclusions, the Wilcoxon signed rank test is further used to show the differences between the block deficiency algorithm and the quadtree algorithm on their search time in each experiment.





\subsubsection*{6.2.1 The experimental results on the pure hands}

First, 1000 randomly generated pure hands are tested to show the performance of the block algorithm, where each hand is tested with 30 random different knowledge bases and they are belonging to the normal distribution. Clearly, this experiment could be effective to avoid the deviation of the experimental results caused by some special knowledge bases for the hand. Table \ref{tab4} shows the experimental results of the block algorithm on the pure hands with the various knowledge bases, including the accuracy rate, the average search time, the ratio of the average search time compared with the quandtree algorithm, and the statistical comparison results based on the Wilcoxon signed rank test (the same below).



\begin{table}
\begin{center}
\caption{\label{tab4} The experimental results of the block algorithm on the pure hands}
\scalebox{0.45}[0.7]{
\begin{tabular}{|c| c| c| c| c| c| c| c|}
\noalign{\vskip 1mm}
\hline \multirow{The number of tile in}  & \multirow{The number of the hand}  & \multicolumn{2}{c|}{Accuracy rate} & \multicolumn{4}{c|}{Computational efficiency} \\
       \cline{3-8}
       ~ & ~ & Quandtree  & Block  &\multicolumn{2}{c|}{Average calculation time in seconds} &Average calculation time ratio & Statistical results\\
       \cline{5-6}
       the knowledge base & (100000) & algorithm & algorithm & Quadtree algorithm & Block algorithm & (Quadtree algorithm/Block algorithm)& (Statistic indicator/ P-value)\\

\hline   [0, 5)  &  4767    & - & 98.72\% & $8.63\times 10^{-2}$ & $1.31\times 10^{-2}$  & $6.58\times 10^{0}$ & 0/0\\
\hline   [5, 10)  &  8923  & - & 99.97\% & $6.05\times 10^{-1}$ & $2.96\times 10^{-2}$  & $2.04\times 10^{1}$ & 0/0\\
\hline   [10, 15)  &  9635  & - & 100\% & $1.32\times 10^{0}$ & $4.01\times 10^{-2}$  & $3.29\times 10^{1}$ & 0/0 \\
\hline   [15, 22]  &  6675  & - & 100\% & $2.20\times 10^{0}$ & $4.48\times 10^{-2}$  & $4.90\times 10^{1}$ & 0/0  \\
\hline total&   -    & - & -     & $1.11\times 10^{0}$ & $3.37\times 10^{-2}$  & $3.28\times 10^{1}$ & 0/0 \\
\hline
\end{tabular}}
\end{center}
\end{table}

From Table \ref{tab4}, we can be seen that the block algorithm has the same search results with the quandtree algorithm on the almost hands, and a faster search efficiency on all cases. In detail, for the search results, the block algorithm just has the error result when the number of tile in the knowledge base (denoted by \emph{nKB}) is in [0, 5) and [5, 10), and the corresponding accuracy rates for them are  $98.72\%$ and $99.97\%$, respectively. Moreover, for the search efficiency, the block algorithm and the quandtree algorithm have $6.58\times 10^{0}$, $2.04\times 10^{1}$, $3.29\times 10^{1}$ and $4.90\times 10^{1}$ in term of the ratio of their average time on the hands with \emph{nKB} in the range of [0, 5), [5, 10), [10, 15) and [15, 22], respectively. Thus, the block algorithm has better search efficiency than the quandtree algorithm. Meanwhile, according to the ratio of the average search time in the Table \ref{tab4}, one can find that the search efficiency of the block algorithm gradually enhances as the \emph{nKB} increases. This might be because the more tiles in the knowledge base, the less invalid combinations in the hand, then reducing the number of {\qd}s in each block. Furthermore, from the statistical results in the Table \ref{tab4}, one can see that the P value is 0 for all cases. So, the computational efficiency of the block algorithm is significantly better than that of the quandtree algorithm. Therefore, the block algorithm has a more search performance than the quandtree algorithm for the pure hand.



\subsubsection*{6.2.2 The experimental results on the hands with two colours}


Moreover, 1000 randomly generated hands with two colours are also tested to show the performance of the block algorithm, where each hand is tested with 100 random different knowledge bases and they are belonging to the normal distribution. Table \ref{tab5} shows the experimental results of the block algorithm on the above hands with the various knowledge bases.

\begin{table}
\begin{center}
\caption{\label{tab5} The experimental results of the block algorithm on the hands with two colours}
\scalebox{0.45}[0.7]{
\begin{tabular}{|c| c| c| c| c| c| c| c|}
\noalign{\vskip 1mm}
\hline \multirow{The number of tile in}   & \multirow{The number of the hand}  & \multicolumn{2}{c|}{Accuracy rate} & \multicolumn{4}{c|}{Computational efficiency} \\
       \cline{3-8}
       ~ & ~ & Quandtree  & Block  &\multicolumn{2}{c|}{Average calculation time in seconds} &Average calculation time ratio & Statistical results\\
       \cline{5-6}
       the knowledge base & (100000) & algorithm & algorithm & Quadtree algorithm & Block algorithm & (Quadtree algorithm/Block algorithm)& (Statistic indicator/ P-value)\\

\hline   [0, 10)  &  9963    & - & 77.31\% & $1.51\times 10^{-2}$ & $5.33\times 10^{-4}$  & $2.83\times 10^{1}$ & 0/0\\
\hline   [10, 20)  &  18798  & - & 99.17\% & $6.90\times 10^{-2}$ & $9.15\times 10^{-4}$  & $7.54\times 10^{1}$ & 0/0\\
\hline   [20, 30)  &  25350  & - & 100\% & $1.56\times 10^{-1}$ & $1.07\times 10^{-3}$  & $1.46\times 10^{2}$ & 0/0 \\
\hline   [30, 40)  &  23646  & - & 100\% & $2.75\times 10^{-1}$ & $1.16\times 10^{-3}$  & $2.37\times 10^{2}$ & 0/0  \\
\hline   [40, 50)  &  15734   & - & 100\% & $3.82\times 10^{-1}$ & $1.22\times 10^{-3}$  & $3.12\times 10^{2}$ & 0/0 \\
\hline   [50, 58]  &  6509    & - & 100\% & $4.57\times 10^{-1}$ & $1.22\times 10^{-3}$  & $3.75\times 10^{2}$ & 0/0 \\
\hline total&   -    & - & -     & $2.09\times 10^{-1}$ & $1.04\times 10^{-3}$  & $2.00\times 10^{2}$ & 0/0 \\
\hline
\end{tabular}}
\end{center}
\end{table}

From Table \ref{tab5}, we can see that the block algorithm obtains the same search results with the quandtree algorithm for most hands, and has a smaller search time with two orders of magnitude in all cases. In detail,
the block algorithm just has $77.31\%$ and $99.17\%$ in term of the accuracy rates when \emph{nKB} is in [0, 10) and [10, 20) respectively, and has $2.83\times 10^{1}$, $7.54\times 10^{1}$, $1.46\times 10^{2}$, $2.37\times 10^{2}$, $3.12\times 10^{2}$ and $3.75\times 10^{2}$ in term of the ratio of their average time on the hands with \emph{nKB} in the range of [0, 10), [10, 20), [20, 30), [30, 40), [40, 50) and [50, 58], respectively.  Meanwhile, according to the ratio of the average search time in the Table \ref{tab5}, one can find that the search efficiency of the block algorithm is gradually improved as the \emph{nKB} increases. The reason for this might be that as \emph{nKB} increases, the tiles in the hand are more likely to form a valid combination with the knowledge base, the reducing the number of {\qd}s in each block. Furthermore, from the statistical results in the Table \ref{tab5}, one can see that the P value is 0 for all cases, such that the block algorithm has a significantly difference with the quandtree algorithm. Thus, the block algorithm is a more promising algorithm for these cases.


\subsubsection*{6.2.3 The experimental results on the hands with three colours}

Finally, to show the performance of the block algorithm, 1000 randomly generated hands with three colours are further tested, and each hand is tested with 100 random different knowledge bases being under the normal distribution. Table \ref{tab6} shows the experimental results of the block algorithm on the above hands with the various knowledge bases.


\begin{table}
\begin{center}
\caption{\label{tab6}  The experimental results of the block algorithm on the hands with three colours}
\scalebox{0.45}[0.7]{
\begin{tabular}{|c| c| c| c| c| c| c| c|}
\noalign{\vskip 1mm}
\hline \multirow{The number of tile in}   & \multirow{The number of the hand}  & \multicolumn{2}{c|}{Accuracy rate} & \multicolumn{4}{c|}{Computational efficiency} \\
       \cline{3-8}
       ~ & ~ & Quandtree  & Block  &\multicolumn{2}{c|}{Average calculation time in seconds} &Average calculation time ratio & Statistical results\\
       \cline{5-6}
       the knowledge base & (100000) & algorithm & algorithm & Quadtree algorithm & Block algorithm & (Quadtree algorithm/Block algorithm)& (Statistic indicator/ P-value)\\

\hline   [0, 10)  &  4966    & - & 62.77\% & $3.13\times 10^{-3}$ & $2.36\times 10^{-4}$  & $1.33\times 10^{1}$ & $3.00\times 10^{0}$/0\\
\hline   [10, 20)  &  8151  & - & 86.66\% & $1.77\times 10^{-2}$ & $3.50\times 10^{-4}$  & $5.07\times 10^{1}$ & 0/0\\
\hline   [20, 30)  &  11407  & - & 99.68\% & $2.97\times 10^{-2}$ & $4.01\times 10^{-4}$  & $7.40\times 10^{1}$ & 0/0 \\
\hline   [30, 40)  &  14519  & - & 100\% & $5.05\times 10^{-2}$ & $4.23\times 10^{-4}$  & $1.19\times 10^{2}$ & 0/0  \\
\hline   [40, 50)  &  15842   & - & 99.97\% & $8.09\times 10^{-2}$ & $4.50\times 10^{-4}$  & $1.80\times 10^{2}$ & 0/0 \\
\hline   [50, 60)  &  15297    & - & 100\% & $1.11\times 10^{-1}$ & $4.58\times 10^{-4}$  & $2.42\times 10^{2}$ & 0/0 \\
\hline   [60, 70)  &  12611     & - & 100\% & $1.39\times 10^{-1}$ & $4.69\times 10^{-4}$  & $2.97\times 10^{2}$ & 0/0 \\
\hline   [70, 80)  &  9454    & - & 100\% & $1.66\times 10^{-1}$ & $4.74\times 10^{-4}$  & $3.50\times 10^{2}$ & $4.17\times 10^{3}$/0\\
\hline   [80, 94]  &  7753     & - & 100\% & $1.90\times 10^{-1}$ & $4.80\times 10^{-4}$  & $3.97\times 10^{2}$ & $8.30\times 10^{4}$/0 \\
\hline total&   -    & - & -     & $9.01\times 10^{-2}$ & $4.30\times 10^{-4}$  & $2.10\times 10^{2}$ & 0/0 \\
\hline
\end{tabular}}
\end{center}
\end{table}

From Table \ref{tab6}, we can see that the block algorithm obtains the same search results with the quandtree algorithm for most hands, and has a faster search efficiency than the quandtree algorithm in all cases. In detail, the block algorithm just has $62.77\%$, $86.66\%$, $99.68\%$ and $99.97\%$ in term of the accuracy rates when \emph{nKB} is in [0, 10), [10, 20), [20, 30) and [40, 50) respectively, and has a more and more larger ratio of the average search time on the hands when \emph{nKB} is gradually increased.  Moreover, according to the ratio of the average search time and the statistical results in the Table \ref{tab6}, one can see that the search efficiency of the block algorithm is better than the quandtree algorithm, and their differences are very significant. Therefore, the block algorithm has a more promising performance than the quandtree algorithm for these cases.

Overall, according to the above descriptions and analysis, one can see that the block algorithm has a similar search performance with the quandtree algorithm for the various hands, and has a significantly faster search efficiency than the quandtree algorithm. Then, the block algorithm has a more promising performance to evaluate the deficiency of one hand. The reason for these might be that the block decomposition in the block algorithm for one hand could effectively reduce the search space, and the various types of all decompositions are only used to calculate the deficiency of the hand, such that the computation cost of the block algorithm could be further degraded. Therefore, the block algorithm is more promising algorithm than the quandtree algorithm.




==> pic/block.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,444); %set diagram left start at 0, and has height of 444

%Shape: Rectangle [id:dp8409799724899254] 
\draw   (23,60) -- (93,60) -- (93,103) -- (23,103) -- cycle ;
%Shape: Rectangle [id:dp15282104665102514] 
\draw   (26,124) -- (96,124) -- (96,167) -- (26,167) -- cycle ;
%Shape: Rectangle [id:dp6336479570664548] 
\draw   (28,287) -- (98,287) -- (98,330) -- (28,330) -- cycle ;
\draw   (104,67) -- (134,82) -- (104,97) -- (119,82) -- cycle ;
\draw   (105,129) -- (135,144) -- (105,159) -- (120,144) -- cycle ;
\draw   (103,295) -- (133,310) -- (103,325) -- (118,310) -- cycle ;
\draw   (265,111) -- (295,126) -- (265,141) -- (280,126) -- cycle ;
\draw   (265,271) -- (295,286) -- (265,301) -- (280,286) -- cycle ;
%Shape: Brace [id:dp631138713569422] 
\draw   (316,99) .. controls (311.33,98.91) and (308.95,101.19) .. (308.86,105.86) -- (308.67,115.32) .. controls (308.54,121.98) and (306.14,125.26) .. (301.47,125.17) .. controls (306.14,125.26) and (308.4,128.64) .. (308.27,135.31)(308.33,132.31) -- (308.14,141.86) .. controls (308.05,146.53) and (310.33,148.91) .. (315,149) ;
%Shape: Brace [id:dp14455728275814228] 
\draw   (394,147) .. controls (398.66,146.79) and (400.89,144.36) .. (400.68,139.7) -- (400.44,134.18) .. controls (400.15,127.52) and (402.33,124.09) .. (406.99,123.88) .. controls (402.33,124.09) and (399.85,120.86) .. (399.55,114.2)(399.68,117.2) -- (399.31,108.68) .. controls (399.1,104.02) and (396.67,101.79) .. (392,102) ;

%Shape: Brace [id:dp020533902010329674] 
\draw   (315,178) .. controls (310.33,177.91) and (307.95,180.19) .. (307.86,184.86) -- (307.67,194.32) .. controls (307.54,200.98) and (305.14,204.26) .. (300.47,204.17) .. controls (305.14,204.26) and (307.4,207.64) .. (307.27,214.31)(307.33,211.31) -- (307.14,220.86) .. controls (307.05,225.53) and (309.33,227.91) .. (314,228) ;
%Shape: Brace [id:dp6397411076722055] 
\draw   (393,226) .. controls (397.66,225.79) and (399.89,223.36) .. (399.68,218.7) -- (399.44,213.18) .. controls (399.15,206.52) and (401.33,203.09) .. (405.99,202.88) .. controls (401.33,203.09) and (398.85,199.86) .. (398.55,193.2)(398.68,196.2) -- (398.31,187.68) .. controls (398.1,183.02) and (395.67,180.79) .. (391,181) ;

%Shape: Brace [id:dp7867920753009139] 
\draw   (319,262) .. controls (314.33,261.91) and (311.95,264.19) .. (311.86,268.86) -- (311.67,278.32) .. controls (311.54,284.98) and (309.14,288.26) .. (304.47,288.17) .. controls (309.14,288.26) and (311.4,291.64) .. (311.27,298.31)(311.33,295.31) -- (311.14,304.86) .. controls (311.05,309.53) and (313.33,311.91) .. (318,312) ;
%Shape: Brace [id:dp847940825538362] 
\draw   (397,310) .. controls (401.66,309.79) and (403.89,307.36) .. (403.68,302.7) -- (403.44,297.18) .. controls (403.15,290.52) and (405.33,287.09) .. (409.99,286.88) .. controls (405.33,287.09) and (402.85,283.86) .. (402.55,277.2)(402.68,280.2) -- (402.31,271.68) .. controls (402.1,267.02) and (399.67,264.79) .. (395,265) ;

\draw   (413,112) -- (443,127) -- (413,142) -- (428,127) -- cycle ;
\draw   (417,188) -- (447,203) -- (417,218) -- (432,203) -- cycle ;
\draw   (416,276) -- (446,291) -- (416,306) -- (431,291) -- cycle ;
%Shape: Rectangle [id:dp8419440563844531] 
\draw   (27,203) -- (97,203) -- (97,246) -- (27,246) -- cycle ;
\draw   (102,211) -- (132,226) -- (102,241) -- (117,226) -- cycle ;
\draw   (263,190) -- (293,205) -- (263,220) -- (278,205) -- cycle ;
%Shape: Brace [id:dp555148193361775] 
\draw   (462,101) .. controls (457.33,100.91) and (454.95,103.19) .. (454.86,107.86) -- (454.67,117.32) .. controls (454.54,123.98) and (452.14,127.26) .. (447.47,127.17) .. controls (452.14,127.26) and (454.4,130.64) .. (454.27,137.31)(454.33,134.31) -- (454.14,143.86) .. controls (454.05,148.53) and (456.33,150.91) .. (461,151) ;
%Shape: Brace [id:dp9813252832830746] 
\draw   (517,152) .. controls (521.67,152) and (524,149.67) .. (524,145) -- (524,138) .. controls (524,131.33) and (526.33,128) .. (531,128) .. controls (526.33,128) and (524,124.67) .. (524,118)(524,121) -- (524,110) .. controls (524,105.33) and (521.67,103) .. (517,103) ;
%Shape: Brace [id:dp9749163779815015] 
\draw   (465,177) .. controls (460.33,176.91) and (457.95,179.19) .. (457.86,183.86) -- (457.67,193.32) .. controls (457.54,199.98) and (455.14,203.26) .. (450.47,203.17) .. controls (455.14,203.26) and (457.4,206.64) .. (457.27,213.31)(457.33,210.31) -- (457.14,219.86) .. controls (457.05,224.53) and (459.33,226.91) .. (464,227) ;
%Shape: Brace [id:dp760126473179177] 
\draw   (520,228) .. controls (524.67,228) and (527,225.67) .. (527,221) -- (527,214) .. controls (527,207.33) and (529.33,204) .. (534,204) .. controls (529.33,204) and (527,200.67) .. (527,194)(527,197) -- (527,186) .. controls (527,181.33) and (524.67,179) .. (520,179) ;

%Shape: Brace [id:dp9001040765199608] 
\draw   (465,265) .. controls (460.33,264.91) and (457.95,267.19) .. (457.86,271.86) -- (457.67,281.32) .. controls (457.54,287.98) and (455.14,291.26) .. (450.47,291.17) .. controls (455.14,291.26) and (457.4,294.64) .. (457.27,301.31)(457.33,298.31) -- (457.14,307.86) .. controls (457.05,312.53) and (459.33,314.91) .. (464,315) ;
%Shape: Brace [id:dp40384757212514466] 
\draw   (520,316) .. controls (524.67,316) and (527,313.67) .. (527,309) -- (527,302) .. controls (527,295.33) and (529.33,292) .. (534,292) .. controls (529.33,292) and (527,288.67) .. (527,282)(527,285) -- (527,274) .. controls (527,269.33) and (524.67,267) .. (520,267) ;

%Shape: Brace [id:dp7564569919569586] 
\draw   (542,294) .. controls (546.67,293.97) and (548.99,291.63) .. (548.96,286.96) -- (548.57,223.42) .. controls (548.53,216.75) and (550.84,213.41) .. (555.51,213.38) .. controls (550.84,213.41) and (548.49,210.09) .. (548.45,203.42)(548.47,206.42) -- (548.03,134.96) .. controls (548,130.29) and (545.66,127.97) .. (540.99,128) ;
%Shape: Brace [id:dp5428510144012235] 
\draw   (578,188) .. controls (573.33,187.91) and (570.95,190.19) .. (570.86,194.86) -- (570.67,204.32) .. controls (570.54,210.98) and (568.14,214.26) .. (563.47,214.17) .. controls (568.14,214.26) and (570.4,217.64) .. (570.27,224.31)(570.33,221.31) -- (570.14,230.86) .. controls (570.05,235.53) and (572.33,237.91) .. (577,238) ;
%Shape: Brace [id:dp028833681451243542] 
\draw   (610,239) .. controls (614.67,239) and (617,236.67) .. (617,232) -- (617,225) .. controls (617,218.33) and (619.33,215) .. (624,215) .. controls (619.33,215) and (617,211.67) .. (617,205)(617,208) -- (617,197) .. controls (617,192.33) and (614.67,190) .. (610,190) ;

%Flowchart: Decision [id:dp1873121851217534] 
\draw   (589.5,55) -- (639,81.5) -- (589.5,108) -- (540,81.5) -- cycle ;

%Right Arrow [id:dp3745631753755052] 
\draw   (584.73,183.09) -- (583.55,140.74) -- (577.47,140.91) -- (588.84,112.34) -- (601.79,140.23) -- (595.71,140.4) -- (596.89,182.75) -- cycle ;


% Text Node
\draw (318,98) node [anchor=north west][inner sep=0.75pt]    {$ \begin{array}{l}
combined\ \\
\ qdcmps\\
\ of\ suite\ b
\end{array}$};
% Text Node
\draw (317,178) node [anchor=north west][inner sep=0.75pt]    {$ \begin{array}{l}
combined\ \\
\ qdcmps\\
\ of\ suite\ c
\end{array}$};
% Text Node
\draw (321,262) node [anchor=north west][inner sep=0.75pt]    {$ \begin{array}{l}
combined\ \\
\ qdcmps\\
\ of\ suite\ d
\end{array}$};
% Text Node
\draw (463,185.4) node [anchor=north west][inner sep=0.75pt]    {$ \begin{array}{l}
types\ of\ \\
\ suite\ c
\end{array}$};
% Text Node
\draw (463,273.4) node [anchor=north west][inner sep=0.75pt]    {$ \begin{array}{l}
types\ of\ \\
\ suite\ d
\end{array}$};
% Text Node
\draw (574,196.4) node [anchor=north west][inner sep=0.75pt]    {$ \begin{array}{l}
types\ \\
\ of\ T
\end{array}$};
% Text Node
\draw (563.84,70.24) node [anchor=north west][inner sep=3pt]   [align=left] {\  decide};
% Text Node
\draw (53,172.4) node [anchor=north west][inner sep=0.75pt]    {$\vdots $};
% Text Node
\draw (36,362) node [anchor=north west][inner sep=0.75pt]   [align=left] {blocks};
% Text Node
\draw (139,65.4) node [anchor=north west][inner sep=0.75pt]    {$\Bigl\{qdcmps\ of\ b_{1}\Bigr\}$};
% Text Node
\draw (52,76.4) node [anchor=north west][inner sep=0.75pt]    {$b_{1}$};
% Text Node
\draw (142,128.4) node [anchor=north west][inner sep=0.75pt]    {$\Bigl\{qdcmps\ of\ b_{2}\Bigr\}$};
% Text Node
\draw (142,293.4) node [anchor=north west][inner sep=0.75pt]    {$\Bigl\{qdcmps\ of\ b_{\ell }\Bigr\}$};
% Text Node
\draw (51,133.4) node [anchor=north west][inner sep=0.75pt]    {$b_{2}$};
% Text Node
\draw (55,299.4) node [anchor=north west][inner sep=0.75pt]    {$b_{\ell }$};
% Text Node
\draw (113,172.4) node [anchor=north west][inner sep=0.75pt]    {$\vdots $};
% Text Node
\draw (191,172.4) node [anchor=north west][inner sep=0.75pt]    {$\vdots $};
% Text Node
\draw (142,204.4) node [anchor=north west][inner sep=0.75pt]    {$\Bigl\{qdcmps\ of\ b_{s}\Bigr\}$};
% Text Node
\draw (54,215.4) node [anchor=north west][inner sep=0.75pt]    {$b_{s}$};
% Text Node
\draw (54,257.4) node [anchor=north west][inner sep=0.75pt]    {$\vdots $};
% Text Node
\draw (110,257.4) node [anchor=north west][inner sep=0.75pt]    {$\vdots $};
% Text Node
\draw (187,257.4) node [anchor=north west][inner sep=0.75pt]    {$\vdots $};
% Text Node
\draw (460,109.4) node [anchor=north west][inner sep=0.75pt]    {$ \begin{array}{l}
types\ of\ \\
\ suite\ b
\end{array}$};
% Text Node
\draw (128,352) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{101.37pt}\setlength\topsep{0pt}
quasi-decompositions
\begin{center}
of individual blocks
\end{center}

\end{minipage}};
% Text Node
\draw (299,341) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{77.56pt}\setlength\topsep{0pt}
combined quasi-\\decompositions
\begin{center}
of three suites
\end{center}

\end{minipage}};
% Text Node
\draw (456,342) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{48.09pt}\setlength\topsep{0pt}
\begin{center}
types of \\individual \\suites
\end{center}

\end{minipage}};


\end{tikzpicture}


==> pic/maxsum.tex <==
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,513); %set diagram left start at 0, and has height of 513

%Shape: Diamond [id:dp24719655985292976] 
\draw   (335,47) -- (365.5,69.5) -- (335,92) -- (304.5,69.5) -- cycle ;

%Straight Lines [id:da21994663203888432] 
\draw    (335,92) -- (335,112) ;
%Shape: Ellipse [id:dp4158531498698175] 
\draw   (312,131.75) .. controls (312,120.84) and (322.3,112) .. (335,112) .. controls (347.7,112) and (358,120.84) .. (358,131.75) .. controls (358,142.66) and (347.7,151.5) .. (335,151.5) .. controls (322.3,151.5) and (312,142.66) .. (312,131.75) -- cycle ;
%Straight Lines [id:da13399703983514888] 
\draw    (361,148.5) -- (404.54,189.14) ;
\draw [shift={(406,190.5)}, rotate = 223.03] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da42528855646657115] 
\draw    (335,152) -- (335.96,195.5) ;
\draw [shift={(336,197.5)}, rotate = 268.74] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da13415894278690033] 
\draw    (314,148.5) -- (276.49,182.16) ;
\draw [shift={(275,183.5)}, rotate = 318.09000000000003] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp02758838896163529] 
\draw   (312,198) -- (362,198) -- (362,238) -- (312,238) -- cycle ;

%Straight Lines [id:da4669220110095267] 
\draw    (335,239) -- (335,259) ;
%Shape: Ellipse [id:dp6741397791430257] 
\draw   (319,280) .. controls (319,271.44) and (326.16,264.5) .. (335,264.5) .. controls (343.84,264.5) and (351,271.44) .. (351,280) .. controls (351,288.56) and (343.84,295.5) .. (335,295.5) .. controls (326.16,295.5) and (319,288.56) .. (319,280) -- cycle ;
%Straight Lines [id:da8173168944915432] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (355,286.5) -- (423.18,317.67) ;
\draw [shift={(425,318.5)}, rotate = 204.57] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da0015340437156845521] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (334.03,298.5) -- (334.96,342.58) ;
\draw [shift={(335,344.58)}, rotate = 268.79] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da10611579309109098] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (319,280) -- (269.69,311.43) ;
\draw [shift={(268,312.5)}, rotate = 327.49] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Diamond [id:dp18326819751493884] 
\draw   (336.5,344.58) -- (379,372.04) -- (336.5,399.5) -- (294,372.04) -- cycle ;
%Shape: Diamond [id:dp8765032449870997] 
\draw   (263.5,314.58) -- (304,342.04) -- (263.5,369.5) -- (223,342.04) -- cycle ;
%Shape: Diamond [id:dp4397448577915206] 
\draw   (435,321.58) -- (483,348.04) -- (435,374.5) -- (387,348.04) -- cycle ;
%Shape: Rectangle [id:dp7429319280889517] 
\draw   (405,191) -- (456,191) -- (456,229.5) -- (405,229.5) -- cycle ;

%Shape: Rectangle [id:dp7634010451800641] 
\draw   (236,185) -- (282,185) -- (282,219.5) -- (236,219.5) -- cycle ;

%Straight Lines [id:da896816429507548] 
\draw    (559,272.5) -- (614,273.46) ;
\draw [shift={(616,273.5)}, rotate = 181.01] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da8149506355261844] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (557.03,349.5) -- (620,348.53) ;
\draw [shift={(622,348.5)}, rotate = 539.12] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Shape: Diamond [id:dp026651665348577325] 
\draw   (581,43) -- (611.5,65.5) -- (581,88) -- (550.5,65.5) -- cycle ;

%Shape: Rectangle [id:dp33638367539776914] 
\draw   (561,134.5) -- (611,134.5) -- (611,161.5) -- (561,161.5) -- cycle ;


% Text Node
\draw (320,126) node [anchor=north west][inner sep=0.75pt]    {$\max$};
% Text Node
\draw (327,270.4) node [anchor=north west][inner sep=0.75pt]    {$\Sigma $};
% Text Node
\draw (314,362.94) node [anchor=north west][inner sep=0.75pt]    {$T[ t/ s_{i}]$};
% Text Node
\draw (339,156.4) node [anchor=north west][inner sep=0.75pt]    {$t_{j}$};
% Text Node
\draw (338,308.4) node [anchor=north west][inner sep=0.75pt]    {$s_{i}$};
% Text Node
\draw (238,332.94) node [anchor=north west][inner sep=0.75pt]    {$T[ t/ s_{1}]$};
% Text Node
\draw (413,339.94) node [anchor=north west][inner sep=0.75pt]    {$T[ t/ s_{27}]$};
% Text Node
\draw (294,306.4) node [anchor=north west][inner sep=0.75pt]    {$\cdots $};
% Text Node
\draw (365,306.4) node [anchor=north west][inner sep=0.75pt]    {$\cdots $};
% Text Node
\draw (284,273.4) node [anchor=north west][inner sep=0.75pt]    {$s_{1}$};
% Text Node
\draw (382,277.4) node [anchor=north west][inner sep=0.75pt]    {$s_{27}$};
% Text Node
\draw (388,160) node [anchor=north west][inner sep=0.75pt]    {$t_{14}$};
% Text Node
\draw (285,150) node [anchor=north west][inner sep=0.75pt]    {$t_{1}$};
% Text Node
\draw (298,174.4) node [anchor=north west][inner sep=0.75pt]    {$\cdots $};
% Text Node
\draw (357,174.4) node [anchor=north west][inner sep=0.75pt]    {$\cdots $};
% Text Node
\draw (414,202) node [anchor=north west][inner sep=0.75pt]    {$T/ t_{14}$};
% Text Node
\draw (580,254.4) node [anchor=north west][inner sep=0.75pt]    {$t_{j}$};
% Text Node
\draw (547,284) node [anchor=north west][inner sep=0.75pt]   [align=left] {discard tile};
% Text Node
\draw (612,284.4) node [anchor=north west][inner sep=0.75pt]    {$t_{j}$};
% Text Node
\draw (554,359) node [anchor=north west][inner sep=0.75pt]   [align=left] {draw tile};
% Text Node
\draw (610,361) node [anchor=north west][inner sep=0.75pt]    {$s_{i}$};
% Text Node
\draw (584,335) node [anchor=north west][inner sep=0.75pt]    {$s_{i}$};
% Text Node
\draw (321,209.4) node [anchor=north west][inner sep=0.75pt]    {$T/ t_{j}$};
% Text Node
\draw (245,193.74) node [anchor=north west][inner sep=0.75pt]    {$T/ t_{1}$};
% Text Node
\draw (329,61.4) node [anchor=north west][inner sep=0.75pt]    {$T$};
% Text Node
\draw (575,57.4) node [anchor=north west][inner sep=0.75pt]    {$T$};
% Text Node
\draw (556,97) node [anchor=north west][inner sep=0.75pt]   [align=left] {a 14-tile};
% Text Node
\draw (539,174) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{78.14pt}\setlength\topsep{0pt}
\begin{center}
a 14-tile with \\one tile removed
\end{center}

\end{minipage}};
% Text Node
\draw (570,138.4) node [anchor=north west][inner sep=0.75pt]    {$T/ t_{j}$};
\end{tikzpicture}


==> temp/pricai21draft.tex <==
\section{Introduction}
\label{S:1}
From the very beginning of AI research,  from checker \cite{Samuel59}, chess \cite{shannon1988programming}, Go \cite{Silver+16} to poker \cite{bowling2015heads} and StarCraft II \cite{VinyalsBCMDCCPE19}, games have played as test-beds of many AI techniques and ideas. In the past decades, we have seen AI programs that can beat best human players in perfect information games including checker, chess and Go, where players know everything occurred in the game before making a decision. Imperfect information games are more challenging. Important progress has been made in solving the two-player heads-up  Texas hold'em poker \cite{bowling2015heads,BrownS17}. 

Another recent breakthrough \cite{li2020suphx} attacks the more popular and more complicated Mahjong game, which is a tile-based multiplayer game played worldwide. The game is played with a set of 144 tiles based on Chinese characters and symbols (see Figure~\ref{fig:mjtiles})  and has many variations in tiles used, rules, and scores \cite{Wiki_mahjong}. Each player begins with a hand of 13 tiles and, in turn, players draw and discard tiles until they complete a legal hand. Suphx, the Mahjong AI from Microsoft Research Asia \cite{li2020suphx}, is designed for Japanese Mahjong based on deep reinforcement learning and has demonstrated super-human performance in the Tenhou platform. Another strong Mahjong AI was reported in \cite{MizukamiT15}, where the authors built a computer Mahjong player based on Monte Carlo simulation and opponent models trained with game records. While these achievements are indeed remarkable, they have the common limitations such as poor interpretability and dependency on expensive game records of human expert players. 

In this paper, we initiate a mathematical and knowledge-based AI study of Mahjong, aiming to explore ways of integrating traditional knowledge-based AI with machine learning. This is partially motivated by the fact that Mahjong is a combinatorial game where (a) solutions (i.e., legal hands) have structures which can be exploited and specified as local constraints, and (b) the player's belief or knowledge about the distribution of non-shown tiles (in the other players' hands or the Wall) can be updated as knowledge/belief revision. Theory and practice of knowledge representation and reasoning (KRR) \cite{krhandbook} has provided a plethora of methods, e.g., Bayesian inference, constraint solving and optimisation, belief revision, which can be exploited in the design of Mahjong AI. It is also expected that these knowledge-based methods can be further combined with machine learning methods proposed in \cite{bowling2015heads,BrownS17,li2020suphx}. In particular, the rule-based Mahjong AI can provide the initial batch of self-played game records (which are usually hard or expensive to collect) that are necessary in the machine learning approach.  


%Despite of its extremely popularity, there are very few mathematical or AI research papers which are devoted to the study of the Mahjong game. To our best knowledge, \cite{Cheng18} is the first serious attempt to study the Mahjong game using mathematical (mainly elementary combinatorial theory) techniques.

In this paper, for simplicity, we only consider a very basic and essential version of Mahjong. The other variations can be dealt with analogously. There are three types of tiles used in the basic version of Mahjong:
\begin{itemize}
    \item Bamboos: $B1, B2, ..., B9$, each with four identical tiles
    \item Characters: $C1, C2, ..., C9$, each with four identical tiles
    \item Dots: $D1, D2, ..., D9$, each with four identical tiles
\end{itemize}
In this paper, we call \emph{Bamboo} ($B$), Character ($C$), Dot ($D$) \emph{colours} of the tiles, and write $\M_{0}$ for the set of these tiles, which include in total 108 tiles. 

\begin{figure}[tbp]
    \centering
    \includegraphics[width=0.6\textwidth]{mjtiles.png}
    \caption{Mahjong tiles, from https://en.wikipedia.org/wiki/Mahjong}\label{fig:mjtiles}
    \label{fig:my_label}
\end{figure}

\begin{dfn}
An \emph{eye} is a pair of identical tiles, a \emph{pong} {\rm(}\emph{kong}{\rm)} is a sequence of three {\rm(}four{\rm)} identical tiles. A \emph{chow} is a sequence of three consecutive tiles of the same colour. A \emph{meld} is either a pong or a chow. 
\end{dfn}


In this work, we also need the following non-standard notions.
\begin{dfn}\label{dfn:pmeld}
A \emph{pseudochow} {\rm(}\emph{pchow}{\rm)} is a pair of tiles of the same colour s.t. it becomes a chow if we add an appropriate tile with the same colour. A \emph{pseudomeld} {\rm(}\emph{pmeld}{\rm)} is a pchow or a pair.  We say a tile $c$ \emph{completes} a meld $(ab)$ if $(abc)$ {\rm(}after alphabetic sorting{\rm)} is a meld. Similarly, a pair is completed from a single tile $t$ if it is obtained by adding an identical tile to $t$.
\end{dfn}

For example, $(B3B4B5)$ is a chow, $(C1C1)$ is an eye, $(B7B7B7)$ is a pong, $(D9D9D9D9)$ is a kong, and $(B1B3)$ and $(C2C3)$ are two pchows.


The remainder of this paper is organised as follows. Sec.~2  introduces basic notions related to 14-tiles, and characterises how bad a pure or hybrid 14-tile is in Sec. 3 and 4, respectively. Sec.~5 presents an optimal policy for discarding tiles. A simple rule-based Mahjong AI is presented and evaluated in Sec.~6. The last section concludes the paper with directions for future research. Due to space limitation, all proofs of our results, which are not very difficult, are omitted.

\section{Pure and Hybrid 14-Tiles}

Recall that each player begins with a set of 13 tiles (called her \emph{hand}). Then players may change a tile by either drawing a new tile or robbing a tile, say $t$, discarded by another player if the player has two identical tiles $t$ and wants to consolidate a pong $(ttt)$ or if $t$ completes her 13-hand into a legal hand. %\footnote{In $\mahjong_0$ we assume that kongs play no role in forming legal hands.} 
In this paper, we take the following defined 14-tiles as our object of study. 
\begin{dfn}
\label{dfn:14-tile}
A 14-tile is a sequence $S$ of 14 tiles from $\M_0$. A sequence of tiles is \emph{pure} if they are all of the same colour and is \emph{hybrid} if otherwise.
\end{dfn}
Apparently, no identical tiles can appear more than four times in a 14-tile. To be precise, we often write a tile $t$ as a pair $(c,n)$ s.t. $c \in \{0,1,2\}$ denotes the colour of $t$ and $n$ denotes the number of $t$. Here we assume that $0, 1,2$ denote, respectively, Bamboo, Character, and Dot. For example, $(0,3)$ and $(1,5)$ denote $B3$ and $C5$ respectively. Moreover, we assume that each 14-tile is represented in the standard form in the following sense.

\begin{dfn}
\label{dfn:standard14-tile}
The \emph{standard form} of a {\rm(}hybrid{\rm)} 14-tile is a sequence $H$ of pairs $(c,n)$ with $0\leq c \leq 2$ and $1\leq n \leq 9$. We denote as $H[i]=(c_i,n_i)$ the $(i+1)$-th tile in $H$ and require, for each $0\leq i \leq 13$, that $c_i \leq c_{i+1}$ and $n_i \leq n_{i+1}$ if $c_i = c_{i+1}$.
We require that there are no five identical tiles in $H$.
\end{dfn}

For the purpose of this work, a pure 14-tile of Bamboos is not different from a pure 14-tile of Dots or a pure 14-tile of Characters. Thus we simply write a pure 14-tile as a 14-tuple of integers from 1 to 9 if the colour of the tiles is clear from the context or not important. Formally, we have
\begin{dfn}
A \emph{pure} 14-tile $S$ is a sequence of 14 integers with non-decreasing integer value from 1 to 9 and no value appears more than four times. 
\end{dfn}
Suppose $S$ is a sequence of 14 integers. Write $S[i]$ for the $(i+1)$-th value of $S$ for $0 \leq i \leq 13$, i.e., we assume, as in Python and many other programming languages, that $S[0]$ represents the first entity of $S$. Then $S$ is a pure 14-tile iff:
\begin{itemize}
    \item $S[i] \in \mathbb{N}$ and $1\leq S[i] \leq 9$ for each $0\leq i \leq 13$; and
    \item $S[i] \leq S[i+1]$ for any $0\leq i \leq 12$; and
    \item $S[i] < S[i+4]$ for any $0 \leq i \leq 9$.
\end{itemize}

%\lsj{Consider removing this paragraph.}
%For each pure 14-tile $S$, we define its \emph{set sequence}, written $\sset(S)$, as the subsequence of $S$ obtained by deleting, for each tile $(c,n)$ in $S$, all but the first occurrences of $(c,n)$ in $S$, and define its \emph{residual sequence} as  $\Res(S) \equiv S\setminus \sset(S)$.\footnote{In this paper, we regard a sequence as a set and identical items in the same sequence are considered as different elements in the corresponding set. Thus, suppose $W$ is a subsequence of $V$, $V\setminus W$ denotes the subsequence with items in $W$ removed from $V$.} For example, consider the following pure 14-tile $S$ and its set and residual sequences:
%\begin{align*}
%    S \quad &=\ (1,1,1,2,2,3,3,4,7,7,7, 8,8,9,9) \\
%    \sset(S) &=\ (1,2,3,4,7,8,9) \\
%    \Res(S) & =\ (1,1,2,3,7,7,8,9)
%\end{align*}
%For convenience, we also write these sequences compactly as\\ \quad $S=(111223347778899)$, $\sset(S)=(1234789)$, and $\Res(S)=(11237789)$.

\begin{dfn}
\label{dfn:complete&decomposition}
A 14-tile over $\M_0$ is \emph{legal} or \emph{complete} if it can be decomposed into four melds and one eye. Given a complete 14-tile $T$, a \emph{decomposition} $\pi$ of $T$ is a sequence of five subsequences of $V$ s.t. 
$\pi[4]$ is a pair (the eye) and, for $1\leq i\leq 4$, each $\pi[i-1]$ is a meld.
\end{dfn}
For ease of presentation, we don't regard a hand with seven pairs as complete.
%
\begin{dfn}
\label{dfn:14tile_graph}
Two 14-tiles $S, T$ over $\M_0$  are \emph{neighbours} if $S[i] = T[i]$ holds for all but exactly one $i \in [0,13]$. The 14-tile graph is the pair $(\mathcal{T},E)$, where $\mathcal{T}$ is the collection of all 14-tiles and two 14-tiles $S,T$ are connected by an edge if $S,T$ are neighbours. The distance between two 14-tiles $S,T$ is the length of a shortest path from $S$ to $T$ in the 14-tile graph. 
\end{dfn}
%
\begin{dfn}
\label{dfn:dfncy}
The \emph{deficiency number} \rm{(}or simply \emph{deficiency}\rm{)} of a 14-tile $S$ is defined recursively:
\begin{itemize}
    \item A 14-tile has deficiency 0 if it is complete;
    \item A 14-tile has deficiency 1 if it is not complete but has a complete neighbour;
    \item In general, for $\ell\geq 0$, a 14-tile has deficiency $\ell+1$ if it has no deficiency smaller than or equal to $\ell$ and it has a neighbour which has deficiency $\ell$.
\end{itemize}
If the deficiency of $S$ is $\ell$, we write $\dfncy(S) = \ell$.
\end{dfn}

For example, the following 14-tile is complete and, thus, has deficiency 0.
\begin{align}\label{mjsol1}
H &= (B1B2B2B3B3B4B7B7B7)(C1C1)(D4D5D6)
\end{align}
In this example, we have the following decomposition
\begin{align*}
    \pi &= (B1B2B3)(B2B3B4)(B7B7B7)(D4D5D6)(C1C1).
\end{align*}

A 14-tile $T$ is often not complete. The deficiency number of $T$ measures how bad $T$ is by counting the number of necessary tile changes to make it complete. 


In the following two sections, we consider how to compute the deficiency number of a pure and, respectively, a hybrid 14-tile. 

\section{Deficiency of Pure 14-Tiles}
%\lsj{Shorten this section!}

In this section we prove the following theorem.
\begin{theorem}\label{thm:pure}
Any pure 14-tile has deficiency less than or equal to 3.
\end{theorem}
To prove this theorem, we need to make several simple observations. First, there exists a pure 14-tile that has deficiency 3:
\begin{align}\label{14-tile_dfncy=3}
%V & = (B1 B1 B2 B2 B5 B5 B6 B6 B8 B8B8B8 B9B9)
V & = (1 1 2 2 5 5 6 6 8 888 99)
\end{align}
Indeed, this pure 14-tile has only one meld, viz. $(888)$. To get four melds, we need to replace some tiles with others (with the same colour). Since each tile can be used to construct at most one meld or one eye, we need at least 3 tile changes to obtain four melds. Suppose without loss of generality this pure 14-tile is in colour $B$. Then we may replace both $B2$ with $B4$, obtaining two chows $(B4B5B6)$, and replace one $B8$ with $B9$, obtaining a pong $(B9B9B9)$.  %This example leads to the following fact.
%Thus we have
%\begin{lemma}\label{fact<=3}
%There exists a pure 14-tile with deficiency 3.
%\end{lemma}
By Definition~\ref{dfn:pmeld}, a pair of tiles say $(Bi,Bj)$ is a pmeld if $|j-i| \leq 2$. In what follows, we assume that a meld (kong) can also be counted as a pmeld (pong).

%\begin{lemma}
%\label{fact2}
%Any four tiles of the same colour contain a pmeld. 
%\end{lemma}
%\begin{proof}
%Suppose $V=(abcd)$ is a set of four tiles of the same colour and $1\leq a \leq b \leq c \leq d \leq 9$. If $a=b$ or $b=c$ or $c=d$, we have a pair and thus a pmeld. Now, suppose $1\leq a < b < c < d \leq 9$. It's easy to see that $b-a > 2$, $c-b > 2$, and $d-c > 2$ cannot happen in the same time. Thus $V$ has at least one pmeld.
%\end{proof}
The following notion of `disjoint' pmelds/melds is important.
\begin{dfn}
\label{dfn:disjoint}
Suppose $V$ is a sorted tuple of $k$ $(3\leq k\leq 14)$ tiles of the same colour. We say two sorted pmelds $(uv),(xy)$ contained in $V$ are \emph{disjoint}, if $(uv)$ and $(xy)$ are not identical pairs and there exist indices $0\leq i<j<p<q<k$ s.t. $u=V[i], v=V[j], x=V[p]$ and $y=V[q]$. Similarly, two sorted melds $(abc)$ and $(xyz)$ are \emph{disjoint} if there exist indices $0\leq i_1<i_2<i_3<i_4<i_5<i_6<k$ s.t. $a=V[i_1], b=V[i_2], c=V[i_3], x=V[i_4], y=V[i_5]$, and $z=V[i_6]$. 
\end{dfn}
In the same sense, we can also define when a meld and a pmeld are disjoint, and when $V$ contains three or more disjoint pmelds.

Consider the tuple $W=(1248)$ of four tiles of the same colour. It has two pmelds, viz. (12) and (24), but they are not disjoint in our sense. Furthermore, consider $V=(111158)$. It has two identical pairs $(11)$, which are in a sense competing with each other and cannot both be useful in forming a legal hand. That's why we don't consider them as disjoint pmelds.   
%How about five tiles of the same colour? Do we always have two disjoint pmelds? Here by `disjoint' we mean the two pmelds/melds do not share the same (occurrence of a) tile, but they may have tiles that are identical. 


%For six tiles of the same colour, we have the following result.
%
%\begin{lemma}
%\label{fact3}
%Suppose $V$ is a tuple of six tiles of the same colour. If $V$ contains no kong, then $V$ contains at least two disjoint pmelds. If, in addition, $V$ contains six pairwise different tiles, then $V$ contains a chow and a disjoint pchow or contains three disjoint pchows. 
%\end{lemma}
%\begin{proof}
%Suppose $V=(abcdef)$ has no kong. Here we don't assume that $V$ is sorted. First, we consider the case when $V$ contains at least one pair, say $a=b$. By Lemma~\ref{fact2}, there is a pmeld in $(cdef)$, which cannot be $(aa)$ as $V$ has no kong. Thus $V$ contains two disjoint pmelds if it has no kong.  

%Second, suppose $V$ contains six different tiles and $a<b<c<d<e<f$. It is easy to see that, among $b-a$, $c-b$, $d-c$, $e-d$, and $f-e$, there exist at most one that is greater than 2. In fact, this is because
%$8= 9-1 \geq f-a = (f-e) + (e-d) + (d-c) + (c-b) + (b-a)\geq 1 + 1 + 1 + 1 + 1 = 5$ and $8 < 3+3+1+1+1 = 9$. %This shows that $V$ contains one chow and a pchow or contains three disjoint pchows in this case.
%\end{proof}

The following result shows that if $V$ contains two disjoint melds, then it can be completed within two tile changes.
\begin{proposition}\label{prop0}
If $V$ contains two disjoint melds, then $\dfncy(V)\leq 2$.
\end{proposition}
%\begin{proof}
%The proof is not difficult but lengthy, see~\ref{sec:appendix1}.
%\end{proof}

%For any pure 14-tile $V$, recall that $\sset(V)$ is the set sequence of $V$, containing all different tiles in $V$, and $\Res(V)\equiv V\setminus\sset(V)$, containing all the rest tiles. 
%For example, for the 14-tile in Eq.~\eqref{14-tile_dfncy=3}, $\sset(V) = (125689)$.

%\begin{proof}[Proof of Theorem~\ref{thm:pure}]
%We prove Theorem~\ref{thm:pure} case by case.
%
%Suppose $|\sset(V)|=8$ or $|\sset(V)|=9$. 
%We have at least two chows in $\{(123),(456),(789)\}$. By Proposition~\ref{prop0}, we know $\dfncy(V)\leq 2$.
%
%Suppose $|\sset(V)| = 4$ or $|\sset(V)| = 5$. Then  $V$ contains at least two different pongs in both cases. By Proposition~\ref{prop0}, we have $\dfncy(V) \leq 2$.
%
%Suppose $|\sset(V)|=6$ or $|\sset(V)|=7$. If $V$ contains two or more disjoint melds, by Proposition~\ref{prop0}, we know $\dfncy(V)\leq 2$.
%
%Suppose $|\sset(V)|=7$ and $V$ does not contain two disjoint melds. Let $\sset(V)$ $=(abcdefg)$ with $a<b<c<d<e<f<g$. It is easy to see that $\sset(V)$ contains one chow.  We note that $\Res(V)$ must contain a pair, this is because, otherwise, we have  $\Res(V)=\sset(V)$ and $V$ shall contain two chows. Thus $V$ consists of one kong or pong and at least four different pairs. Clearly, $V$ can be completed within three tile changes in this case. That is, $\dfncy(V)\leq 3$.
%
%Suppose $|\sset(V)|=6$ and $V$ does not contain two disjoint melds. In particular, it has no two differnt pongs. Let $\sset(V)=(abcdef)$. This implies that $V$ consists of one kong and five different pairs. Clearly, $V$ can be completed within three tile changes, by completing any three pairs into pongs. This shows $\dfncy(V)\leq 3$.
%\end{proof}


%Note that if, for example, $V=(11115555779999)$, then $\sset(V)=(1579)$ and we need exactly two tile changes to complete $V$.


A simple brute force search shows that the numbers of pure 14-tiles and those have deficiency 0 (i.e., complete),  1, 2, 3 are as follows. 
\begin{itemize}
    \item 118800 valid pure 14-tiles
    \item 13259 complete pure 14-tiles
    \item 91065 pure tiles with deficiency 1
    \item 14386 pure tiles with deficiency 2
    \item 90 pure tiles with deficiency 3 
\end{itemize}
One natural question is, do we have more direct methods to determine the deficiency of a 14-tile by, e.g., examining its structure? This is possible. In particular,  we have the following characterisation for pure 14-tiles with deficiency 3.
\begin{proposition}
\label{lem:7}
For any pure 14-tile $V$, $V$ has deficiency 3 iff either
\begin{itemize}
    \item [\rm (i)] $V$ consists of a kong and 5 different pairs; or
    \item [\rm (ii)] $V$ consists of five different pairs, a pong $(ppp)$ and a single tile $s$, and has a tile $x$ s.t. $(psx)$ {\rm(}after ordering{\rm)} is a chow and $V\setminus(psx)$ contains no chows.
\end{itemize}
\end{proposition}
Note that, by abuse of notation, we regard a sequence as a multi-set and identical items in the same sequence are considered as different elements in the corresponding set. For two sequences $V,W$, $V\setminus W$ denotes the subsequence with items in $W$ removed from $V$. Similar explanations apply to $V\cap W$ and $V\cup W$.

Consider the pure 14-tile $V = (11222344558899)$ as an example. $V$ consists of a pong $(222)$, a single tile $3$ and five pairs $(11)$,  $(44)$, $(55)$, $(88)$, $(99)$. Thus $\dfncy(V)=3$. Note that if we accept seven pairs as a complete hand, then the deficiency of a pure 14-tile is at most 2!


\section{Deficiency of Hybrid 14-Tiles}
When is a hybrid 14-tile $H$ complete? How many tile changes are necessary to complete it if it is not? These questions can be answered by computing the deficiency of $H$. There is one problem: the deficiency of $H$ is defined in a recursive way and, to tell if $\dfncy(H)$ is $k+1$, one need to know in principle all 14-tiles with deficiency $k$. It will be more convenient if we can determine, just like Proposition~\ref{lem:7},  the deficiency of $H$ by analysing its structure directly.

In this section, we present a method for determining if a 14-tile is complete, and show that the worst 14-tiles have deficiency 6 and give a characterisation for these 14-tiles, and then give a direct and efficient method for measuring the `badness' of a hybrid 14-tile $H$, and prove that it is exactly the deficiency of $H$.

\subsection{The best and the worst 14-tiles}

We first show how to decide if a hybrid 14-tile $H$ is complete. For convenience, we introduce the following notations.

\begin{dfn}
\label{dfn:H_b}
Given a hybrid 14-tile $H$, we write $n_b(H)$, $n_c(H)$, and $n_d(H)$ for the numbers of Bamboos, Characters, and Dots in  $H$. We denote by $H_b$, $H_c$, and $H_d$ for, respectively, the subsequences of Bamboos, Characters, and Dots in $H$. 
A hybrid 14-tile $H$ is called a bcd-type 14-tile if $n_b\geq n_c\geq n_d$.
\end{dfn}

For the hybrid 14-tile $H$ in Eq.~\eqref{mjsol1}, we have $H_b=(122334777)$, $H_c=(11)$, and $H_d=(456)$, where we omit the colour symbol $B,C,D$ in $H_b,H_c$ and $H_d$. Since $n_b(H)=9$, $n_c(H)=2$, $n_d(H)=3$, $H$ is not a bcd-type 14-tile. But it is easy to see that every hybrid 14-tile $T$ has a corresponding bcd-type 14-tile $S$ s.t. $S$ and $T$ are identical in essence.

\begin{proposition}
\label{prop:complete_14tile}
A bcd-type 14-tile $H$ is complete iff one of the following conditions is satisfied:
\begin{itemize}
    \item $n_b=14$, $n_c=n_d=0$ and $H$ is a complete pure 14-tile; 
    \item $n_b=12$, $n_c=2$, $n_d=0$, $H_b$ consists of four disjoint melds and $H_c$ consists of a pair;
    \item $n_b=11$, $n_c=3$, $n_d=0$, $H_b$ consists of three disjoint melds and a pair and $H_c$ consists of a meld;
    \item $n_b = 9$, $n_c = 5$, $n_d = 0$, $H_b$ consists of three disjoint melds and $H_c$ consists of a meld and a pair;
    \item $n_b=9$, $n_c=3$, $n_d=2$, $H_b$ consists of three disjoint melds, $H_c$ consists of a meld, and $H_d$ consists of a pair;
    \item $n_b=8$, $n_c=3$, $n_d=3$, $H_b$ consists of two disjoint melds and a pair and each of $H_c$ and $H_d$ consists of a meld;
    \item $n_b=8$, $n_c=6$, $n_d=0$, $H_b$ consists of two disjoint melds and a pair and $H_c$ consists of two disjoint melds; 
    \item $n_b=6$, $n_c=6$, $n_d=2$, each  of $H_b$ and $H_c$ consists of two disjoint melds and $H_d$ consists of a pair;
    \item $n_b=6$, $n_c=5$, $n_d=3$, $H_b$ consists of two disjoint melds, $H_c$ consists of a meld and a pair, and $H_d$ consists of a meld.
    \end{itemize}
\end{proposition}

Knowing how to decide if a hybrid 14-tile is complete, we next present one method for deciding the deficiency number of a hybrid 14-tile.

\begin{lemma}\label{lem:distance}
A 14-tile $H$ has deficiency $\leq k$ iff there exists a sequence of $s\leq k$ 14-tiles $H_1$, $H_2$, ..., $H_s$, s.t. $H_s$ is complete, and $H_i$ is a neighbour of $H_{i-1}$ for every $1\leq i\leq s$, where $H_0 = H$.
\end{lemma}
%Since a tile change from a 14-tile $H$ leads to a neighbour of $H$, we have the following corollary. 
%\begin{coro}\label{coro:1}
%A 14-tile $H$ has deficiency $k$ iff it can be changed into a complete 14-tile by $k$ tile changes but cannot be changed into a complete 14-tile by $k-1$ or less tile changes.
%A 14-tile $H$ has deficiency $\leq k$ iff it can be changed into a complete 14-tile by $\leq k$ tile changes.
%\end{coro}
Indeed, every 14-tile can be completed within six tile changes.
\begin{proposition}
\label{prop:dfncy<=6}
For any 14-tile $H$, the deficiency of $H$ is not greater than 6.
\end{proposition}

For example, the following 14-tile has deficiency 6 as it has only three disjoint pmelds, e.g., $(B1B2)$, $(C2C2)$, and $(D6D8)$.
\begin{align}\label{eq:14-tile_dfncy6}
H &= (B1B1B2B5B8)(C1C2C2C5C8)(D3D6D8D9).
\end{align}

%As proved in Theorem~\ref{thm:pure}, if $H$ is pure, then $\dfncy(H) \leq 3$. Similarly, if at least nine tiles are of the same colour, then the deficiency of $H$ is smaller than 6.  
%\begin{proposition}\label{prop:dfncy<=5}
%Given a 14-tile $H$, if $H_b$ contains 9 tiles, then $\dfncy(H)\leq 5$.
%\end{proposition}
%\begin{proof}
%We show that $H_b$ contains two disjoint melds, or one meld and two disjoint pmelds, or four disjoint pmelds. We discuss this case by case. Note that if $H_b$ contains two pongs, or two disjoint melds, or four disjoint pairs, we are done. 

%Suppose $H_b$ contains only one pong $(aaa)$. By Lemma~\ref{fact3} the remaining 6 tiles contains two pmelds $(bc)$ and $(de)$. Assume $b<c$ and $d<e$. If $a$ completes both $(bc)$ and $(de)$, then we have two chows. If $a$ completes only one of $(bc)$ and $(de)$, we have a pair $(aa)$, a chow and a pmeld. If $a$ completes neither $(bc)$ nor $(de)$, then we can complete $(bc)$ and $(de)$ in two tile changes without violating the constraint that there are no five identical tiles in $\mahjong_0$. 

%Suppose $H_b$ contains no pongs.  If $H_b$ contains only three different pairs, then $H_b$ has the form $(aa)(bb)(cc)$ $(d)(e)(f)$ with $a<b<c$ and $d<e<f$. 
%        \begin{itemize}
%            \item Suppose $e-d \leq 2$ or $f-e \leq 2$. Then we have three pairs and one pmeld. 
%            \item Suppose $e-d>2$ and $f-e>2$. If $(abc)$ is a meld, then we already have at least two melds. If $(abc)$ is not a meld and $(xyz)$ is a meld, where $x,y \in \{a,b,c\}$ and $z \in \{d,e,f\}$, then we have one meld $(xyz)$, one pmeld $(xy)$ and one pair. If there is no meld in $H_b$, since $H_b$ has six different tiles, we can show that there exist $x\in \{a,b,c\}$ and $y,z\in \{d,e,f\}$ s.t. $(yx)$ and $(xz)$ are two pmelds. Together with two other pairs,  we also have four disjoint pmelds in $H_b$.    
%        \end{itemize}

%Suppose $H_b$ contains no pongs and has only two different pairs. Then $\sset(H_b)$ has seven different tiles and thus at least one chow $(def)$ ($d<e<f$). Write $(aa)$ and $(bb)$ for the two pairs in $H_b$, where $a<b$. If $a,b$ are not in $\{d,e,f\}$, then we have one meld and two different pairs. If $a,b$ are both in $\{d,e,f\}$, then $(ab)$ is a pchow. Since there is a pmeld in the other four tiles of $H_b$, we also have one chow and two pmelds in this case. If, for example, $a\in \{d,e,f\}$ but $b\not\in\{d,e,f\}$, then we have one chow $(def)$, one pair $(bb)$, and another pmeld in the remaining four tiles of $H_b$. 

%Suppose $H_b$ has only one pair. Then, since $\sset(H_b)$ has 8 different tiles, there are two disjoint chows in $H_b$.

%This shows that $\dfncy(H) \leq 5$ if $H_b$ contains 9 tiles. 
%\end{proof}
Analogous to the pure case, we could also have a  characterisation of the worst 14-tiles, which is omitted due to space limitation.

%Next, we give a characterisation of the worst 14-tiles. To this end, we need the following notion of worst pure $k$-tiles for $1\leq k \leq 8$: 
%\begin{dfn}
%Let $k$ be an integer between 1 and 8. A \emph{pure $k$-tile} $V$ is a sequence  of integers in $[0,9]$ s.t. no integer appears more than four times and $V[i] \leq V[i+1]$ for any $0\leq i<k-1$.  

%We say a pure $k$-tile $V$ is a worst $k$-tile if 
%\begin{itemize}
%    \item when $1\leq k\leq 3$, $V$ contains no pmelds; 
%    \item when $k=4$ or $k=5$, $V$ contains no meld and contains only one pmeld;
%    \item when $k=6$, $V$ contains at most one meld or up to two disjoint pmelds;
%    \item when $k=7$, $V$ contains up to two disjoint pmelds;
%    \item when $k=8$, $V$ contains at most one meld and a disjoint pmeld, or up to three disjoint pmelds.
%\end{itemize}
%\end{dfn}

%\begin{proposition}\label{prop:dfncy=6}
%For any 14-tile $H$, $\dfncy(H)=6$ iff one of the following situation occurs:
%\begin{itemize}
%    \item [1.] 
%    $n_b(H) = 8$, $n_d(H) = n_c(H) = 3$, $H_c$ and $H_d$ contain no pmeld and $H_b$ is a worst pure 8-tile.
    
%    \item [2.] $n_b(H) = 7$,  $n_c(H) =5$, $n_d(H)=2$, $H_b$ is a worst pure 7-tile and $H_c$ a worst pure 5-tile and $H_d$ has no pmeld.
%    \item [3.] $n_b(H) = 6$,  $n_c(H) =5$, $n_d(H)=3$, $H_b$ is a worst pure 6-tile and $H_c$ a worst pure 5-tile, and $H_d$ has no pmeld.
%   \item [4.] $n_b(H) = n_c(H) =5$, $n_d(H)=4$, $H_b$ and $H_c$ are worst pure 5-tiles and $H_d$ a worst pure 4-tile. 
%\end{itemize} 
%\end{proposition}

%
\subsection{A direct method for measuring the badness of a 14-tile}

While in principle we can determine if the deficiency of a hybrid 14-tile  $\leq k$  by recursively checking if it has a neighbour with deficiency $<\!k$, this is far from efficient. We provide a direct method for measuring the badness of a 14-tile. To this end, we first extend the notion of decomposition to incomplete 14-tiles.
%
\begin{dfn}
Given any 14-tile $T$, a \emph{pseudo-decomposition} {\rm(}\emph{{\pd}}{\rm)} of $T$ is a sequence $\pi$ of five subsequences, $\pi[0],...,\pi[4]$, of $T$ s.t. 
\begin{itemize}
    \item $\pi[4]$ is a pair, a single tile, or empty;
    \item for $0\leq i\leq 3$, each $\pi[i]$ is a meld, a pmeld, a single tile, or empty.
\end{itemize}
For convenience, we write $\pi[5]\equiv T \setminus \bigcup_{i=0}^4 \pi[i]$  for the sequence of remaining tiles.
\end{dfn}

%
\begin{dfn}
\label{dfn:normal_dcmp}
A {\pd} $\pi$ of a 14-tile $T$ is \emph{completable} if there exists a decomposition $\pi^*$ of a complete 14-tile $S$  s.t. $\pi[i]$ is a subsequence of $\pi^*[i]$ for each $0\leq i\leq 3$. If this is the case, we call $S$ a \emph{completion} of $T$ based upon $\pi$. 

A completable {\pd} $\pi$ is \emph{saturated} if no tiles in $\pi[5]$ can be added into $\pi[i]$ for any $0\leq i\leq 3$ to form another completable {\pd}.  
%A {\pd} $\pi$ of $T$ is called \emph{normal} if $\pi$ is saturated and has a completion $S$ which is a closest complete 14-tile of $T$.

The \emph{cost} of a completable {\pd} $\pi$, written $\cost_T(\pi)$,  is the number of necessary tile changes to complete $\pi[4]$ into a pair and complete each $\pi[i]$ into a meld for $0\leq i\leq 3$. If a {\pd} $\pi$ is incompletable, we say it has infinite cost. 
%and write $\cost_T(\pi)=\infty$.
\end{dfn}

A 14-tile $T$ may have many different {\pd}s.  

%The following results will be useful, where we say a {\pd} $\pi_1$ \emph{refines} another {\pd} $\pi_2$ if $\pi_1(i)\supseteq \pi_2(i)$ for any $1\leq i\leq 5$.
%\begin{lemma}\label{lem:saturated}
%Suppose $\pi$ is a {\pd} of a 14-tile $T$. If $\pi$ is completable but not saturated, then there exists a saturated completable {\pd} $\pi^*$ s.t. $\pi^*$ refines $\pi$ and $\cost_T(\pi^*) < \cost_T(\pi)$.
%\end{lemma}
%\begin{proof}
%Suppose $\pi$ itself is not saturated. By definition, there exist $t\in \pi[5]$ and $1\leq i\leq 5$ s.t. $\pi(i)$ is not a meld (a pair) when $i\leq 4$ ($i=5$) and  adding $t$ to $\pi(i)$ results a new completable {\pd} $\pi^*$. Clearly, $\cost_T(\pi^*)=\cost_T(\pi)-1$. If $\pi^*$ is not saturated, then we can further refine it till it is saturated. The conclusion then follows immediately. 
%\end{proof}

%The above lemma shows that we need only consider saturated completable {\pd}s. The next result states that the cost of a {\pd} of $T$ is identical to the distance between $T$ and any completion of $T$ based upon $\pi$. 

%\begin{lemma}
%\label{lem:dcmp-dist}
%Suppose $\pi$ is a saturated completable {\pd} of a 14-tile $T$. Then, for any completion $S$ of $T$ based upon $\pi$, we have $\dist(S,T)=\cost_T(\pi)$.
%\end{lemma}
%\begin{proof}
%Note that any completion $S$ is obtained by filling the `holes' in $\pi$. Since $\pi$ is saturated, these holes cannot be filled by using tiles in $\pi[5]$. Thus, each hole must be filled by a tile change. Therefore, $S$ has distance $\cost_T(\pi)$ with $T$.
%\end{proof}


%The following result shows that, very often, 
%Very often, a saturated {\pd} has no empty subsequences.

%\begin{proposition}\label{prop:normal}
%Suppose $T$ is a 14-tile and $\pi$ is a completable {\pd} which has an empty subsequence. If $\pi[5]$ contains 4 or more tiles or $\pi[4]\not=\varnothing$, then there exists another completable {\pd} $\pi^*$ which has no empty subsequences and $\cost_T(\pi^*) < \cost_T(\pi)$. 
%\end{proposition}
%\begin{proof}
% See \ref{sec:appendix2}.
%\end{proof}
%As a corollary, we have 
%\begin{coro}\label{coro:emptyss}
%Suppose $T$ is a 14-tile and $\pi$ a completable {\pd} with $n\geq 2$ empty subsequences. There exists a completable {\pd} $\pi^*$ s.t. $\cost_T(\pi^*) \leq\cost_T(\pi)-n$.
%\end{coro}


\begin{example}
\label{ex:T9}
Consider the 14-tile 
\begin{align*}%\label{eq:T9}
T &=(B1B1B2B2B2B2B3B3)(C1C2C8)(D2D2D8).
\end{align*}
It is easy to check that the following are all its {\pd}s 
\begin{align*}%\label{eq:D(T9)0}
\pi_0 &= (B1B2B3)(B2B2B2)(B1B3)(D2D2)(D8) \\
%\label{eq:D(T9)1}
\pi_1 &= (B1B2B3)(B1B2B3)(B3)(D2D2)(D8)\\
%\label{eq:D(T9)2}
\pi_2 &= (B1B2B3)(B1B2B3)(C1C2)(D2D2)(B2B2).
\end{align*}
The pmeld $(B1B3)$ in $\pi_0$ cannot be completed, as there are already four $B2$ in $\pi_0$. Both $\pi_1$ and $\pi_2$ are saturated and completable. For examples, $\pi_1$  and $\pi_2$ can be, respectively, completed into 
\begin{align*}
(B1B2B3)(B1B2B3)(B3\underline{B4}\underline{B5})(D2D2\underline{D2})(D8\underline{D8})\\
(B1B2B3)(B1B2B3)(C1C2\underline{C3})(D2D2\underline{D2})(B2B2).
\end{align*}
We have $\cost_T(\pi_1)=4$ and $\cost_T(\pi_2)=2$. Since $\dfncy(T)=2$, $\pi_2$ is a {\pd} with the minimal cost.  
\end{example}
%The deficiency of $T$ is indeed the minimal cost among all {\pd}s of $T$.
\begin{theorem}\label{thm:m-cost}
The deficiency of a 14-tile $T$ is the minimum cost of its {\pd}s: 
\begin{align}
    \dfncy(T) = \min\{\cost_T(\pi) \mid \mbox{$\pi$ is a {\pd} of $T$}\} .
\end{align} 
\end{theorem}

In what follows, we say a {\pd} $\pi$ of a 14-tile $T$ is \emph{minimal} if $\cost_T(\pi) = \dfncy(T)$. We next present an efficient method for determining the deficiency of a 14-tile by constructing such a minimal {\pd} of $T$.

 \subsubsection{Our procedure}
 We construct a quadtree, where each node is denoted by a word $\alpha$ in the alphabet $\Sigma=\{1,2,3,4\}$ and we attach to each $\alpha$ a subsequence $S_\alpha$ of $T$, which denotes the set of tiles remaining to be processed, and a {\pd} $\pi_\alpha$ of $T$, and maintain a queue $Q$ of nodes to be explored and a global current best value $\val$. Initially, the root node, denoted as the empty word $\varepsilon$, is put in $Q$. We define $S_\varepsilon=T$, the {\pd} $\pi_\varepsilon$ with $\pi_\varepsilon[i]=\varnothing$ for $0\leq i\leq 5$, and set $\val=6$, the largest possible deficiency number.
 
% \lsj{Add a figure here to illustrate the procedure?}
 
 Suppose a node $\alpha$ is popped out from the queue $Q$ and suppose $\val$ is the current best value and $S_\alpha$ and $\pi_\alpha$ are,  respectively, the  subsequence and the {\pd} associated with $\alpha$. We \emph{expand} $\alpha$ as follows. Let $a=S_\alpha[0]$ be the first tile in the subsequence $S_\alpha$. We add  up to four child nodes $\alpha1$ to $\alpha4$ under the node $\alpha$. For each $\ell\in\{1,2,3,4\}$, the subsequence $S_{\alpha\ell}$ and the {\pd} $\pi_{\alpha\ell}$ are obtained by \emph{reducing} $S_\alpha$ and \emph{refining} $\pi_\alpha$ respectively. 
 
 \paragraph{Notation}\quad Given a tile $t=(c,n)$, we write $t^+$ ($t^{++}$, resp.) for $(c,n+1)$ ($(c,n+2)$, resp.) as long as $1\leq n\leq 8$ ($1\leq n\leq 7$, resp.); and write $ t^-$ ( $t^{--}$, resp.) for $(c,n-1)$ ($(c,n-2)$, resp.) as long as $2\leq n \leq 9$ ($3\leq n\leq 9$, resp.).
 
 \begin{itemize}
     \item Define $S_{\alpha1}=S_\alpha\setminus (a)$ and $\pi_{\alpha1}=\pi_\alpha$.
     
     \item If $a^+$ or $a^{++}$ is in $S_\alpha$,\footnote{If this is not the case, then this node is not introduced. Similar assumption applies to the other two child nodes.}
     define $S_{\alpha2}=S_\alpha \setminus (aa^+a^{++})$.\footnote{If, for example, $(aa^+a^{++}) \cap S_\alpha=(aa^{++})$, then $S_\alpha \setminus (aa^+a^{++})=S_\alpha \setminus (aa^{++})$.} Suppose $i$  is the first index in $\{0,1,2,3\}$ s.t.  $\pi_\alpha[i]=\varnothing$. Define $\pi_{\alpha2}[i]=(aa^+a^{++})\cap S_\alpha$  and $\pi_{\alpha2}[j]= \pi_\alpha[j]$ for $j\not=i$.\footnote{If $(a^-aa^+)$ is contained in $S$, then this chow shall have been put in some $\pi$ in a previous step when $a^-$ is examined.} 
    
    \item If $(aa)\subseteq S_\alpha$ and $\pi_\alpha[4]$ is empty, define $S_{\alpha3} = S_\alpha \setminus (aa)$ and $\pi_{\alpha3}[4]=(aa)$ and $\pi_{\alpha3}[j]=\pi_\alpha[j]$ for $0\leq j\leq 3$.
    
    
    \item If $(aa)\subseteq S_\alpha$,  define  $S_{\alpha4} = S_\alpha \setminus (aaa)$.
    Suppose $i$ is the first index in $\{0,1,2,3\}$ s.t. $\pi_\alpha[i]=\varnothing$. Define $\pi_{\alpha4}[i]=(aaa)\cap S_\alpha$  and $\pi_{\alpha4}[j]= \pi_\alpha[j]$ for $j\not=i$.
 \end{itemize}
 
For each child node $\alpha\ell$, if $\pi_{\alpha\ell}[i]\not=\varnothing$ for all  $0\leq i\leq 4$,
then we compare the value $\cost_T(\pi_{\alpha\ell})$ with the current best value $\val$, update $\val$ as $\cost_T(\pi_{\alpha\ell})$ if the latter is smaller, and terminate this branch. 

Suppose $\pi_{\alpha\ell}[i]$ is empty for some $i$ but there are no more tiles left to process, i.e., $S_{\alpha\ell}=\varnothing$. We may recycle from $\pi_{\alpha\ell}[5]$ some discarded tiles and put it in some subsequence of $\pi_{\alpha\ell}$ to get a refined completable {\pd}.  Suppose $\pi_{\alpha\ell}[4]\not=\varnothing$ or  $\pi_{\alpha\ell}[5]$ contains four or more tiles. Let $n$ be the number of empty $\pi_{\alpha\ell}[i]$ for $0\leq i\leq 4$. It is not difficult to see that there exists another completable {\pd} $\pi'$ s.t.  $\cost_{T}(\pi') \leq \cost_T(\pi_{\alpha\ell})-n$. We then compare $\cost_T(\pi_{\alpha\ell})-n$ with $\val$ and update $\val$ as  $\cost_T(\pi_{\alpha\ell})-n$ if the latter is smaller, and terminate this branch. 

Suppose $S_{\alpha\ell}=\varnothing$, $\pi_{\alpha\ell}[4]=\varnothing$ and $\pi_{\alpha\ell}[5]$ contains two (three) different tiles $u,v$ ($u,v,w$). We set $\cost=\cost_T(\pi_{\alpha\ell})$ if $T$ contains two kongs $(uuuu)$ and $(vvvv)$ (three kongs $(uuuu)$, $(vvvv)$, and $(wwww)$), and set $\cost=\cost_T(\pi_{\alpha\ell})-1$ otherwise. Then we compare $\cost$ with $\val$ and update $\val$ as  $\cost$ if the latter is smaller, and terminate this branch. 

If $S_{\alpha\ell}\not=\varnothing$ and $\pi_{\alpha\ell}$ has an empty subsequence, then we put $\alpha\ell$ in $Q$. 

After $\alpha$ is expanded, if $Q$ is nonempty and $\val>0$, then we pop out another node $\beta$ from $Q$ and expand $\beta$ as above. The whole procedure stops when either $\val=0$ or $Q=\varnothing$.


%\begin{table}[]
%    \centering
%    \begin{tabular}{c|c|c|c}
%    $\#$meld & $\# \pmeld_1$ & $\#\pmeld_2$ & value \\ \hline
%    0 & $\ell$ & $\geq 5$     &  4 \\
%    0 & $\ell$ & $\leq 4$     & $9-\min(\ell,4)$    \\
%    1 & $\ell$ & $\geq 4$     &  3 \\
%    1 & $\ell$ & $\leq 3$     &  $7-\min(\ell,3)$  \\
%    2 & $\ell$ & $\geq 3$     &  2 \\
%    2 & $\ell$ & $\leq 2$     &  $5-\min(\ell,2)$ \\
%    3 & $\ell$ & $\geq 2$     &  1 \\
%    3 & $\ell$ & $\leq 1$     &  $3-\min(\ell,1)$ \\       
%    4 & $\ell$ & $ 1$     &  0 \\
%    4 & $\ell$ & $0$     &  $\leq 2$ \\
%    \end{tabular}
%    \caption{The value of a temporary decomposition, where $\#meld$ ($\#\pmeld_1$ or $\#\pmeld_2$) denotes the number of melds (pmelds or pemlds with a pair) identified in the decomposition}
%    \label{tab:1}
%\end{table}
%
\section{Decision Making}
Given a 14-tile $H$, we have developed methods for deciding if $H$ is complete, and in case it is not complete, measuring how good or bad it is. The next important task is to decide, in case $H$ is not complete, which tile should the agent discard?

We suppose the agent maintains a  \emph{knowledge base} $\omega$, which contains all her information about the available tiles. For simplicity, we represent $\omega$ as a 27-tuple, where $\omega(c,n)\equiv\omega[9c+n]$ ($0\leq c\leq 2$ and $1\leq n \leq 9$) denotes the number of identical tiles $t=(c,n)$ the agent \emph{believes} to be available. Initially, we have $\omega(c,n) = 4$ for each tile $t=(c,n)$. When all players have their hands, the agent also has her hand $H$ and updates her $\omega$ accordingly as
\begin{align}
\omega(c,n) = 4- \mbox{the number of  $(c,n)$ in $H$}. 
%|\{0\leq i\leq 13 \mid H[i] = (c,n)\}|.
\end{align}
Then she continues to modify $\omega$ according to the process of the game. For example, if one player discards a tile $t=(c,n)$ and no pong is formed from the discard of $t$, then the agent updates her $\omega$ by decreasing by one her $\omega(c,n)$ and leaves the other items unchanged. More advanced techniques will be investigated in future work, where we may record the history of every player, and \emph{reason} about the most likely  distribution (in other players' hands or the Wall) for each tile. 

Suppose the agent has a 14-tile $T$ and her current knowledge base is $\omega$. For simplicity, we write $\norm{\omega}\equiv \sum\{\omega(c,n) \mid 0\leq c\leq 2, 1\leq n\leq 9\}$
%\begin{align}
%\norm{\omega} \equiv \sum\{\omega(c,n) \mid 0\leq c\leq 2, 1\leq n\leq 9\}
%\end{align}
for the number of available tiles and say $\omega$ is empty if $\norm{\omega}=0$.
Our task is to decide which tile she should discard. We associate each tile $t$ in $T$ with a value  
\begin{align}\label{eq:delta}
    \delta_{T,\omega}(t) &= \sum_{0\leq c\leq 2, 1\leq n\leq 9}\Big\{\omega(c,n) \mid \dfncy(T[t/(c,n)]) < \dfncy(T)\Big\}.
\end{align}
Naturally, we change $t$ to an available tile $(c,n)$ only if it is profitable, i.e., if the 14-tile obtained by replacing $t$ with $(c,n)$, written $T[t/(c,n)]$, has a smaller deficiency. For each $t\in T$, $\delta_{T,\omega}(t)$ denotes the number of available tiles $(c,n)$ (identical tiles are counted differently) s.t. $T[t/(c,n)]$ has a smaller deficiency.

After $\delta_{T,\omega}(t)$ is computed for each $t\in T$, we then pick and discard the tile $t\in T$ which has the maximum value (ties are broken arbitrarily), i.e.,
\begin{align}
\label{eq:discard}
    \discard(T,\omega) = \argmax_{t\in T} \delta_{T,\omega}(t).
\end{align}
\begin{example}\label{ex:decision}
Consider the following 14-tile and assume $\omega[i]=1$ for $0\leq i\leq 26$.
\begin{align*}
H &= (.)(C1C1C1C5C6C8C9C9)(D3D3D4D5D5)\\
\omega &= (333411123\   010433411\    101121422)
%
%H &= (B1B1B1B7B8B8B9)(C1C5C5C5)(D5D6D7)\\
%\omega &= (111114403)(111111111)(111111111)
\end{align*}
%Here, for convenience, we assume that for each tile $t=(c,n)$ there is only one identical tile available, i.e., 

%$\omega[i] = 1$ for any $0\leq i \leq 26$. 
Then we have $\dfncy(H)=2$ and $\delta_{H,\omega}=[9,9,9,13,9,19,9,9,14,14,11,14,14]$. In particular, $\delta_{H,\omega}(C8)=19$, $\delta_{H,\omega}(D3)=14$, and $\delta_{H,\omega}(D5)=14$. Thus, according to Eq.~\eqref{eq:discard}, we should discard $C8$. In this case,  changing $C8$ as any of $C4,C5,C6,C7$, $D3,D4,D5,D6$ will decrease the deficiency number from $2$ to $1$.
\end{example}

%T =  [[1, 1], [1, 1], [1, 1], [1, 5], [1, 6], [1, 8], [1, 9], [1, 9], [1, 9], [2, 3], [2, 3], [2, 4], [2, 5], [2, 5]]
%Pg =  []
%KB =  [3, 3, 3, 4, 1, 1, 1, 2, 3, 0, 1, 0, 4, 3, 3, 4, 1, 1, 1, 0, 1, 1, 2, 1, 4, 2, 2]
%dc =  0
%discard 21 value [[[1, 8], 19], [[2, 3], 14], [[2, 5], 14], [[1, 5], 13], [[2, 4], 11], [[1, 1], 9], [[1, 6], 9], [[1, 9], 9]]
%step 2 value [[[2, 3], 0.038], [[2, 5], 0.038], [[1, 8], 0.026], [[2, 4], 0.018], [[1, 5], 0.014], [[1, 1], 0.006], [[1, 9], 0.006], [[1, 6], 0.005]]


Eq.~\eqref{eq:discard} provides a simple, and easy to compute, heuristics for deciding which tile the agent should discard when her goal is to win as early as possible. It is, however, not an optimal policy. The value of a tile also depends on how many tile changes we could have or could afford before the game is finished. %\lsj{Add discussion here. Consider Example~2 again. Suppose our aim is to maximise our chance of winning within 2 tile changes. Then discarding xx seems more profitable.} 
%For example, if $D1$ is replaced with $B7$ in $H$ of Example~\ref{ex:decision} and the knowledge base is $\omega = (111144403\ 111111111\ 111111111)$, then $\dfncy(H)=1$ and $B8$ should be discarded according to  Eq.~\eqref{eq:discard}. This is apparently not optimal as, if we discard $C1$, then, after drawing any of $B5$, $B6$, $B7$ or $B9$, the deficiency becomes 1 again and we should have more chances to win within two or more tile changes. 
Shortly we will see that discarding $D3$ or $D5$ instead could increase the chance of winning within two tile changes. This is partially due to that we have only one $D4$ but four $C7$ (which makes $C8$ more useful) available in the knowledge base.

We first formalise this intuitive idea in terms of step $k$ discard value.

\begin{dfn}
Suppose $T$ is an incomplete 14-tile and  $\omega$ the current knowledge base. 
For any $k>0$, we define the
\emph{step $k$ discard value} of a tile $t\in T$ w.r.t. $\omega$, written  $\dval_k(T,\omega,t)$, as the chance of completing $T$ within $k$ tile changes if $t$ is discarded first.
\end{dfn}
For the special case when $k=1$, $\dval_1(T,\omega,t)$ is indeed the success chance of obtaining a complete 14-tile by replacing $t$ with some available tile. 

The following related notion measures the chance of completing an incomplete 14-tile $T$ within $k$ tile changes.
\begin{dfn}
Suppose $T$ is an incomplete 14-tile and  $\omega$ the current knowledge base. For any $k>0$, the \emph{step $k$ success rate} of $T$ w.r.t. $\omega$ is defined as
\begin{align}
\srate_k(T,\omega) \equiv  \max_{t\in T} \dval_k(T,\omega,t).
\end{align}
In case $T$ is complete, we define $\srate_k(T,\omega)=1$.
\end{dfn}

Clearly, $\srate_k(T,\omega)=0$ if $\dfncy(T)>k$ or %$0<\dfncy(T)\leq k$ but 
$\norm{\omega}=0$. 

We give a recursive method for computing  $\dval_k(T,\omega,t)$. For consistency, we define the \emph{step 0 success rate} of $T$, written $\srate_0(T)$,  as 1 if $T$ is complete and 0 otherwise. Then $\dval_1(T,\omega,t)$ is the weighted sum over all available tiles $(c,n)$ of the chance of obtaining a complete 14-tile  by changing $t$ as $(c,n)$, where the chance of selecting $(c,n)$ to replace $t$ is $\omega(c,n)/\norm{\omega}$. For any $t\in T$, we have 
\begin{align}
\label{eq:val1}
\dval_1(T,\omega,t) &= \sum_{(c,n)\;:\;\omega(c,n)>0} \frac{\omega(c,n)}{\norm{\omega}} \times \srate_0 \big(T[t/(c,n)] \big)
\end{align} 
In case $\omega$ is empty, we have $\dval_1(T,\omega, t)=0$ for any $t\in T$. If $T$ is not complete, the chance of completing $T$ within $k$ tile changes is the weighted sum of the chances of completing $T[t/(c,n)]$ within $k-1$ tile changes over all $(c,n)$ with $\omega(c,n)>0$. Thus we have the following characterisation:
\begin{align*} %\nonumber
   \dval_k(T, \omega, t) &= \sum_{(c,n)\ :\ \omega(c,n)>0} \frac{\omega(c,n)}{\norm{\omega}} \times \srate_{k-1}\big(T[t/(c,n)],\omega\!-\!(c,n)\big)
\end{align*}
for each  $t\in T$, where $\omega\!-\!(c,n)$ is the knowledge base obtained by decreasing $\omega(c,n)$ by 1, as this tile $(c,n)$ becomes unavailable after replacing $t$ with it. 
This gives a recursive method for selecting the tile to discard.
%\vspace*{-5mm}
\subsubsection{The best tile to discard}
Suppose $T$ is an incomplete 14-tile and $\omega$ is a knowledge base with $\norm{\omega}>0$. Then $t = \discard_k(T,\omega)$ is the tile that has the best chance for completing $T$ within $k$ tile changes if we discard $t$ first, where
\begin{align}\label{eq:discard-k}
\discard_k(T,\omega) = \argmax_{t\in T} \dval_{k}(T,\omega,t)
\end{align}
Compared with Eq.~\eqref{eq:discard},  $\discard_k(T,\omega)$ is more precise if $k>\dfncy(T)$. Consider the 14-tile $H$ and $\omega$ of Example~\ref{ex:decision}. We have $\discard_2(H,\omega)=D3$ or $D5$ as $\dval_2(H,\omega,D3)=\dval_2(H,\omega, D5)=0.038$ and $\dval_2(H,\omega,C8)=0.026$. The larger $k$ is the more precise. However, it is worth noting that the calculation of $\discard_k(T,\omega)$ involves in the worse case $(14 \times 26)^k$ completeness check of 14-tiles! 

\section{A Simple Rule-based Mahjong Program} 
%
To demonstrate the applicability of the proposed approach, we implemented a simple rule-based Mahjong program and evaluated its effectiveness on an online Sichuan Mahjong platform. Sichuan Mahjong, also known as ``Battle to the Bloody End", uses the 108 tiles in $\mahjong_0$. %\footnote{See, e.g., http://www.jasonpym.com/blog/2013/11/23/sichuan-mahjong/.} 
Each player selects and fixes a `daque' colour once she has received her first 13 tiles, and no tile with this colour can appear in her valid solution.  

The rule-based Mahjong program contains four major modules: $\checkhu$, $\checkpong$, $\checkkong$, and $\discard$. For illustration purpose, we adopt the strategy of declaring win whenever possible. That is, our $\checkhu$ module is trivial. The rest three modules relies heavily on deficiency calculation. Whenever the player can pong or kong a tile $t=(c,n)$, our agent compares the hands before and after the pong/kong action. Roughly speaking, if she finds that the deficiency does not increase by two, or when there are many tiles in the Wall, then she proceeds to pong or kong. Otherwise, she stands. As for the $\discard$ module, the agent always discards a daque tile if she has one, and, in case she has no daque tiles, selects a tile according to Eq.~\eqref{eq:discard} and discards.

We then evaluate our Mahjong program on the popular WeChat \emph{Happy Mahjong} platform. As the platform provides no interface for Mahjong AI, one author of this paper acts as the `agent' of our Mahjong program. We played ten consecutive games ten times with human players, with 10-game scores of 8, -6, 12, -1, 14, 27, -8, -15, 49, and -11, respectively and a total score of 69 points (each point represents 400 basic points in the game). The results show that our program, though very simple, is at least competitive with average human players. 


\section{Conclusions and Future Work}
Above we described a mathematical and knowledge-based AI approach of the Mahjong game. As demonstrated in our rudimentary rule-based program, this knowledge-based approach is promising and the key notions of deficiency number and knowledge base may play important roles in devising powerful Mahjong programs. 
There are several serious limitations with the current implementation. First, when selecting a tile to discard, we adopt Eq.~\eqref{eq:discard}, instead of Eq.~\eqref{eq:discard-k}. This is because the latter requires too many deficiency calculations or completeness check, which is time-consuming. If we can design a more efficient method for deficiency calculation, then it is desired to look-ahead and use, e.g., $\discard_2(T,\omega)$, to select a tile to discard if $\dfncy(T)\leq 2$. Second, the `badness' of a hand is highly related with the current knowledge base and, hence, the procedure described in Sec.~4.2 should take the knowledge base into consideration. Third, the current form of knowledge base does not reflect the distribution of non-shown tiles in the hands of other players or the Wall, which the agent could (at least partially) infer from previous actions in the game. Fourth, when discarding a tile, we need also estimate if it is dangerous, that is, if it is useful for other players. Future work will devise more powerful Mahjong programs to overcome the above limitations and further develop the framework.

